Moderator: Moderating Text-to-Image Diffusion Models through Fine-grained Context-based Policies

We present Moderator, a policy-based model management system that allows administrators to specify fine-grained content moderation policies and modify the weights of a text-to-image (TTI) model to make it significantly more challenging for users to produce images that violate the policies. In contrast to existing general-purpose model editing techniques, which unlearn concepts without considering the associated contexts, Moderator allows admins to specify what content should be moderated, under which context, how it should be moderated, and why moderation is necessary. Given a set of policies, Moderator first prompts the original model to generate images that need to be moderated, then uses these self-generated images to reverse fine-tune the model to compute task vectors for moderation and finally negates the original model with the task vectors to decrease its performance in generating moderated content. We evaluated Moderator with 14 participants to play the role of admins and found they could quickly learn and author policies to pass unit tests in approximately 2.29 policy iterations. Our experiment with 32 stable diffusion users suggested that Moderator can prevent 65% of users from generating moderated content under 15 attempts and require the remaining users an average of 8.3 times more attempts to generate undesired content.

==> 0424-discussion.tex <==
expand function too complex
 no $
 set default value


Fig 2 and 3 too small font
    syntax error
    Fig 2 not understandable

Figure font too small

Discussion rewrite
    Computation cost
    no tech base
    millions and billions

Limitations can not completely remove

Section:

Self-reverse fine-tuning
Policy expansion


==> parts/p1-intro-backup.tex <==

%\begin{figure}[htb!]
%\centering
%\includegraphics[width=0.5\textwidth]{figs/fig-%ExampleForConceptPermission.pdf}
%\caption{Only keep the left one and make it bigger. Besides, the fighting one looks ok. we do not need to moderate them. Find a better example. Received}
%\label{fig:exp_example}
%\end{figure}

\begin{figure}[htb!]
\centering
\includegraphics[width=0.5\textwidth]{figs/fig-example-fight2PuppyFight.pdf}
\caption{\sysname\ allows administrators to transform a genAI model into a moderated version based on specified policies. For instance,  an administrator may specify \textit{moderate(man, puppy) when(fighting)} to mitigate the violent imagery. The resulting model substitutes the man with puppies in the context of "furious fighting" for relevant prompts.}
\label{fig:teaser}
\end{figure}

\section{Introduction}

Imagine a future marketplace where model creators can sell their custom AI models to the public. Users may download these models onto their smartphones or personal computers~\cite{OpenAIEx58:online}. Yet, to align with regional regulations and consider teenage users, marketplace administrators will need to implement additional moderation layers, similar to how social media platforms moderate users' posts today~\cite{singhal2023sok}.
In this paper, we focus on the challenges around moderating the output of diffusion models, which can generate photo-realistic images given any text input~\cite{Rombach_2022_CVPR}. 


While many diffusion model services have begun moderating their outputs, existing methods can only moderate content in a coarse and isolated manner. On one hand, most services employ a rule-based keyword lookup method to identify whether the input text contains forbidden phrases from a predefined list~\cite{}, and deny requests if the resulting images include inappropriate or offensive material~\cite{}. 
However, these methods can only moderate content in an all-or-nothing manner, leading to mistakes where benign content is mistakenly blocked or bad content is mistakenly allowed~\cite{Safeimag31:online}. 
On the other hand, Stable Diffusion supports negative prompts, which allows users to specify prompts to avoid (e.g., naked, sexy, nudity) during image generation~\cite{}. More recently, researchers also proposed multiple model editing methods~\cite{gandikota2023erasing,schramowski2023safe} to erase a specific concept. 
But, these methods typically target a single content category at a time~\cite{}. 


To comprehend the content moderation requirements for generative AI (genAI) models, we compared them to social media platforms, examining which social media content moderation guidelines~\cite{singhal2023sok} fit within the content of genAI.
Our analysis yielded three key observations (\S\ref{sec:analogy}). 
First, genAI content moderation requires a context parameter. For example, Facebook does not always remove "content that focuses on depiction of ribs, collar bones, thigh gaps, hips, concave stomach, or protruding spine or scapula", but only takes action "when shared together with terms associated with eating disorders"~\cite{Suicidea20:online}. Second, genAI content moderation requires multiple levels of mitigation, such as blocking the whole image or pixelating a partial area~\cite{Dangerou7:online}. 
Third, content moderation needs are subject to change. For instance, a marketplace might need to prohibit content from terrorist organizations or individuals, and this list may be updated periodically. 
% Additionally,  user groups might require  content moderation rules.


Based on these insights, we then designed \sysname, a system that can transform a Stable Diffusion model into a moderated version based on a set of fine-grained policies specified by administrators. Figure~\ref{fig:teaser} illustrates how a model moderated by \sysname\ replaces men with puppies in the context of "furious fighting" to mitigate the violent imagery. 


The fundamental challenge of \sysname\ is to build a policy enforcement system in the open-vocabulary setting, as users of genAI might input unpredictable prompts, and the model could produce unforeseen image content. To address this, we formulated the moderation policies formally as \textit{moderate(\textcolor{yellow}{A}, \textcolor{green}{B}) when(\textcolor{red}{C}) unless(\textcolor{blue}{D})}, which specifies the goal of \textcolor{yellow}{A} with \textcolor{green}{B} within the context of \textcolor{red}{C}, but allowing an exception in a scenario \textcolor{blue}{D}. \textcolor{yellow}{A}, \textcolor{green}{B}, \textcolor{red}{C} and \textcolor{blue}{D} can be an arbitrary nouns specified by the administrators.

% genAI users may prompt the model in many unexpected ways and the model may output the unexpected image content. To tackle this issue, we first formulated the moderation policies formally as \textit{moderate(\textcolor{yellow}{A}, \textcolor{green}{B}) when(\textcolor{red}{C}) unless(\textcolor{blue}{D})}, which specifies the goal of replacing \textcolor{yellow}{A} with  \textcolor{green}{B}, in context of \textcolor{red}{C}), while allowing an exception (\textcolor{blue}{D}). 
% allows administrators to moderate the output of a stable diffusion model by specifying arbitrary concepts and associated contexts.

% The core of \sysname\ is a fine-grained control system. \sysname\ allows users with a fundamental system primitive, denoted as \textit{moderate(\textcolor{yellow}{A}, \textcolor{green}{B}) when(\textcolor{red}{C}) unless(\textcolor{blue}{D})}, which serves as the instrument for the customizing moderation policies ( \textcolor{yellow}{A}, \textcolor{green}{B}, \textcolor{red}{C} and \textcolor{blue}{D} represent concepts).

Each instantiation of the `moderate' primitive method imparts its specific policy, the enforcement of which is achieved through the mechanism of Task Arithmetic \cite{ilharco2022editing}. Each such `moderate' primitive is compiled into a combination of task vectors. Task vectors, in this context, are responsible for delineating and obliterating the mapping relationships between `the concept' and `the generated image'. Remarkably, the creation of task vectors is executed in a manner entirely devoid of manual intervention, adhering to a data-free paradigm.


In order to ensure the efficacy of each task vector, \sysname\ employs an LLM-based concept expansion. This query expansion process serves to express the abstract concepts, subsequently formulating a set of highly effective prompts for the task vectors. Additionally, \sysname\ offers a robust conflict policy validation mechanism founded on heuristic principles.

To enhance the accessibility and usability of the system, \sysname\ provides a user-friendly web-based interface, offering a seamless and intuitive means for users to interact with the system.


We conducted comprehensive experiments to validate the design of \sysname. First, we provide an evaluation adjusting different scales of task vectors, finetune steps, and finetune image numbers to find the optimal microbenchmarks for \sysname\ to achieve quick and effective moderation. We also evaluate system overhead and time cost for \sysname\ to prove the efficiency of \sysname\ to apply a moderate policy. To mitigate the potential side effects of combining multiple task vectors, we provide several solutions and find out the best one. We explore the effectiveness of controlling concept granularity using arithmetic, providing fine-grained concept control to support fine-grained moderate primitive system in \sysname\. Furthermore, we show the results of different moderate primitive results provided by \sysname. At last, we evaluate \sysname\ on moderating multiple concepts, and show that \sysname\ can effectively apply moderate policies and moderate concepts.




In summary, we make the following contributions:
\begin{enumerate}
    \item A comprehensive examination of content moderation methods used in social networks compared to genAI, identifying three requirements for fine-grained content moderation: contextual moderation, multi-level mitigation, and dynamic moderation.
    \item A structured policy design, represented as \textit{moderate(\textcolor{yellow}{A}, \textcolor{green}{B}) when(\textcolor{red}{C}) unless(\textcolor{blue}{D})}, which allows administrators to specify open-vocabulary moderation policies formally. 
    \item  A low-cost and generalizable enforcement system that can transform a model into a moderated version based on policies specified by administrators. 
    % \item An end-to-end open-source prototype implementation\footnote{The software will be made available post paper publication.} of \sysname\ integrated with Stable Diffusion. 
\end{enumerate}

% \sysname\ that can run across multiple platforms


% \sysname\ that can run across multiple platforms\footnote{The software will be made available post paper publication}.

%At the core of \sysname\ is a 1. Basic System Primitive. Open vocabulary. Task vectors. 
%1.a. Self-data. 
%1.b. Query expansion to transform the abstract concepts. 
%1.c. Single concept → Multiple concepts. 


%1. Fine-grained control. Moderate When Unless. 
%2.a Formulate the content moderation policies. 
%2.b Enforce the policies through Task Arithmetic
%2.c



% low-cost and generalizable permission 

% 3. Our proposal. Cite interfaces. 
% Admins can specify an arbitrary concept. The input and output. The rest of the papers describes three key innovations in making this system possible, 


% 4. Challenge 1: Open vocabulary. The cost and scalability + open vocabulary. Self-censorship in the model. => Self-generated data. => time latency. 
% 4.1 

% 5. Challenge 2: Simultaneous concepts. Interference. However, training with self-generated data has a challenge. The variances will increase. When we have multiple concepts active at the same time. 

% 6. Challenge 3: What does content moderation mean? A diverse set of operations. Replace, 

%7. Evaluation. a) microbenchmark b) cost. \& system latency. c) moderation effectiveness. 



% Stable diffusion models. 
 % The parents may want to have some level of parental controls to the model, a la to today's parent control feature in the smart phone. 

% \begin{figure}[htb!]
% \centering
% \includegraphics[width=\columnwidth]{figs/cp-interface.JPG}
% \caption{Permission interfaces.}
% \label{fig:permissioninterface}
% \end{figure}

% Challenges: 


% Content creation companies apply these models to facilitate the painting creation, automatically image edit and text content generation.


%Zico's paper. Training from scratch. However, very expensive. Not scalable. The open vocabulary nature of LLMs make it very hard to do XXX. 




%\par In this paper, we present \sysname\, a system that allows system administrators to moderate the content of an open source generative AI model, Stable Diffusion using a network-based permission interface. At the core of \sysname\ is  a low-cost and generalizable system primitive to moderate content in stable diffusion models. 

%\par First, \sysname\ will use original pretrained stable diffusion model to generate toxic images. We use 11 toxic concepts in \sysname\ for stable diffusion to generate. Furthermore, to ensure \sysname\ can cover most of the related concepts of the target concepts, \sysname\ use query expansion to explore more related concepts of the target concepts. \sysname\ will use the generated image to finetune the original pretrained stable diffusion model.
%\par Then, \sysname\ will use the model interpotation between each concept's finetuned model and original pretrained model to create unique task vector for each toxic concept.
%\par At last, a network-based permission interface is provided by \sysname\ to enable efficient content moderation of stable diffusion. Each node in the network represents a toxic concept \sysname\ can moderate. The moderation of each concept can affect the quality of generated image of nearby node's concept.
%\par We evaluate the efficiency and performance of \sysname\ to see if it can effectively remove toxic concept due to permission interface's grant. The experiment results demonstrate that \sysname\ can achieve efficient content moderation in stable diffusion.



%\par Recent generative AI have attracted people's attention due to their good quality of generated content. However, the raise of generative AI presents an important challenge. During the training period of such generative AI model, numerous toxic or unethical contents may be learned by it. As a consequence, generative AI can produce unethical content.

%\par Previous industry applications have appiled NSFW filter, a conventional approach to filter the unethical output of generative AI. However, numerous approaches to defeat it. 

%Zico's paper. Training from scratch. However, very expensive. Not scalable. The open vocabulary nature of LLMs make it very hard to do XXX. 


%In this paper, we present \sysname, a system that allows system administrators to moderate the content of an open source generative AI model, Stable Diffusion.
%Imagine that a user may obtain a language model from a public market, and download the model to their smart phone. The parents may want to have some level of parental controls to the model, a la to today's parent control in the smart phone. 

%At the core of \sysname\ is  a low-cost and generalizable system primitive to moderate content in stable diffusion models. 


%\par Previous work weak point:
%\begin{itemize}
%    \item Easy to bypass
%    \item Hard to scale
%\end{itemize}

%\par In this paper, 




%\haojian{Paper outline: }

%1. Background: task vectors through fine-tuning (query expansion)
%2. The Open vocabulary challenge. => Input is open vocabulary | output is open vocabulary. | 
%2. self-regulation
%3. On-the-fly Approximate Permission interface (Network-based control). 


%1. We want to add permission to an arbitrary concept (Open-vocabulary challenge): Training from scratch. Minus it. => State of the art (David's paper: (a) Create a prompt (b) generate imagines (c) use prompt + images to fine-tune the image. Reverse gradient decent. Stackable. )  


%2. Simultaneous permissions without interference: https://github.com/prateeky2806/ties-merging. Task vectors. 
%- 8 concepts. 


%T_1: prompt:gun -> image:gun
%T_2: prompt:gun -> image:gun with mosaic

%3. Mosaic: Target image generations; => Manual Mark; => Concept replacement. 
%https://arxiv.org/abs/2212.04089. 
%1. Fine-tuning dataset size + concept size + scale =>


%TODO: 

%1. Concept diversity. a. objects (gun, breast,), b. activity (killing, mass shooting, intercourse..), c. ***limitation: style

%=> Movie rating. => Concept permission.

%2. Prompt. 

==> parts/p2-2-background.tex <==

%\haojian{Should explain the threat model first before explaining the background. The threat model helps us narrow down the problem. We will need to explain why we chose to modify the weights. }\peiran{Added more descriptions about threat model and why modify model weight}

\section{Background}

\haojian{This section does not work well. Sec. 3.1 and Sec. 3.2 can be briefed in the background. We should cover them in the related work as well. And Sec. 3.3 can go to the runtime section.}

This section provides essential background about model editing and machine unlearning which serves as the technical foundation of \sysname. Since we need to moderate the TTI models through the moderation of their model parameters, two types of model parameter moderation are taken into consideration:

\sssec{Machine unlearning.} Machine unlearning is used to mitigate the potential risk of privacy leakage and copyright infringement in TTI models. In machine unlearning, assuming we have a pretrained model, then some private data within the training data is required to be deleted from the model parameter. We wish the modified model to perform the same as the model trained only using the unprivate data. The most direct method is to retrain a new model without the private, however, such approaches will bring unnecessary costs. Thus machine unlearning is proposed to solve this problem. Machine unlearning can achieve the deletion of the private data in model weight space without huge retraining costs. This aligns with our model moderation requirements.

\sssec{Model editing.} Unlike machine unlearning, model editing aims to replace or add knowledge within model weight space. The research of model editing originates from LLM's need to replace wrong or out-of-date knowledge, news, etc., with right or new knowledge. To avoid heavy training costs, model editing enables developers to slightly edit model parameters to change the model's knowledge without retraining. This aligns with our model moderation requirements as well.

==> parts/p99-archived.tex <==
\begin{table*}[]
\resizebox{\textwidth}{!}{%
\begin{tabular}{|p{2.5cm}|M{1.6cm}|M{1.6cm}|M{1.6cm}|M{1.6cm}|M{1.6cm}|M{1.6cm}|M{1.6cm}|}
\hline
Platform & Dream Studio & Playground & GetImg.AI & leonardo.ai & dezgo & Picso & Stablebility.AI \\ \hline \hline

\rowcolor{gray!10}
Horror & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} \\
%\hline
Abuse & \textcolor[RGB]{0,220,0}{\XSolidBrush} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor[RGB]{0,220,0}{\XSolidBrush} & \textcolor[RGB]{0,220,0}{\XSolidBrush} \\
% \hline
\rowcolor{gray!10}
Gore & \textcolor[RGB]{0,220,0}{\XSolidBrush} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor[RGB]{0,220,0}{\XSolidBrush} & \textcolor[RGB]{0,220,0}{\XSolidBrush} \\
% \hline
Violence & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor[RGB]{0,220,0}{\XSolidBrush} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor[RGB]{0,220,0}{\XSolidBrush} \\
% \hline
\rowcolor{gray!10}
Sexual Content & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} \\
% \hline
Self-Harm & \textcolor[RGB]{0,220,0}{\XSolidBrush} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor[RGB]{0,220,0}{\XSolidBrush} & \textcolor[RGB]{0,220,0}{\XSolidBrush} \\
% \hline
\rowcolor{gray!10}
Piracy & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} \\
% \hline
Illegal Activities & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} \\
% \hline
\rowcolor{gray!10}
Disinformation & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} \\
% \hline
Unlimited Jokes & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} \\
% \hline
\rowcolor{gray!10}
Defamation & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} \\
% \hline
Discrimination/Bias & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} \\
% \hline
\rowcolor{gray!10}
Insulting Beliefs & \textcolor[RGB]{0,220,0}{\XSolidBrush} & \textcolor[RGB]{0,220,0}{\XSolidBrush} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor[RGB]{0,220,0}{\XSolidBrush} \\
% \hline
Creating Conflicts & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} \\
% \hline
\rowcolor{gray!10}
Political Propaganda & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} \\
% \hline
Terrorism & \textcolor{red}{\Checkmark} & \textcolor[RGB]{0,220,0}{\XSolidBrush} & \textcolor[RGB]{0,220,0}{\XSolidBrush} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor[RGB]{0,220,0}{\XSolidBrush} \\
% \hline
\rowcolor{gray!10}
Children Harm & \textcolor[RGB]{0,220,0}{\XSolidBrush} & \textcolor[RGB]{0,220,0}{\XSolidBrush} & \textcolor[RGB]{0,220,0}{\XSolidBrush} & \textcolor[RGB]{0,220,0}{\XSolidBrush} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor[RGB]{0,220,0}{\XSolidBrush} \\
%\hline
Privacy Breaches & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} \\
\rowcolor{gray!10}
Violation of public order and morals & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} \\
%\hline
Threatening national unity and sovereignty & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} \\
\hline \hline
\end{tabular}%
}
\caption{We summarize 7 popular GenAI online platforms. According to the card sorting results we do in Table. \ref{tab:what+why}, we test all the 7 GenAI platforms to see if they can generate certain types of harmful content.}
\label{tab:genAIPolicy}
\end{table*}

% \begin{table*}[]\large
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{|l|p{2.5cm}|p{2.5cm}|p{2.5cm}|p{2.5cm}|p{2.5cm}|p{2.5cm}|}
% \hline
% Harm Content Type                       & Twitter[1] & Meta[2] & Youtube[3] & TikTok[4] & Instagram[5] & Reddit[6] \\ \hline \hline
% Misinformation                          & \Checkmark         & \Checkmark             & \Checkmark       & \Checkmark      &\XSolidBrush      & \Checkmark      \\ \hline
% Violence                                & \Checkmark         & \Checkmark             & \Checkmark       & \Checkmark      &\XSolidBrush      &\XSolidBrush   \\ \hline
% Violent Content (Terrorism, Militarism) & \Checkmark         & \Checkmark             & \Checkmark       & \Checkmark      &\XSolidBrush      &\XSolidBrush   \\ \hline
% Hate Behavior (Discrimination)          & \Checkmark         & \Checkmark             & \Checkmark       & \Checkmark      & \Checkmark         & \Checkmark      \\ \hline
% Bully \& Harassment                        & \Checkmark         & \Checkmark             & \Checkmark       & \Checkmark      & \Checkmark         & \Checkmark      \\ \hline
% Adult Nudity                            & \Checkmark         & \Checkmark             & \Checkmark       & \Checkmark      &\XSolidBrush      &\XSolidBrush   \\ \hline
% Illegal Items and Service               & \Checkmark         & \Checkmark             & \Checkmark       &\XSolidBrush   & \Checkmark         & \Checkmark      \\ \hline
% Abuse \& Exploitation                   & \Checkmark         & \Checkmark             &\XSolidBrush    &\XSolidBrush   &\XSolidBrush      &\XSolidBrush   \\ \hline
% Self-harm                               & \Checkmark         & \Checkmark             &\XSolidBrush    &\XSolidBrush   & \Checkmark         &\XSolidBrush   \\ \hline
% Child sex \& abuse                      & \Checkmark         & \Checkmark             & \Checkmark       & \Checkmark      & \Checkmark         &\XSolidBrush   \\ \hline
% Graphic content (Bloody, Gore, Horror)  & \Checkmark         & \Checkmark             & \Checkmark       & \Checkmark      &\XSolidBrush      & \Checkmark      \\ \hline
% Copyright                               & \Checkmark         & \Checkmark             & \Checkmark       & \Checkmark      & \Checkmark         &\XSolidBrush   \\ \hline
% Personal Privacy                        & \Checkmark         & \Checkmark             &\XSolidBrush    &\XSolidBrush   &\XSolidBrush      & \Checkmark      \\ \hline
% Weapon Content                          &\XSolidBrush      &\XSolidBrush          & \Checkmark       &\XSolidBrush   &\XSolidBrush      &\XSolidBrush   \\ \hline
% \hline
% %References 
% %& \multicolumn{6}{p{2.5cm}|}{\begin{tabular}[c]{@{}l@{}}
% %[1]\href{https://help.twitter.com/zh-cn/rules-and-policies/twitter-rules}{Twitter Rules and Policies}\\
% %[2]\href{https://transparency.fb.com/zh-cn/policies/community-standards/}{Facebook Community Standards}\\
% %[3]\href{https://support.google.com/youtube/topic/2803176}{Youtube Policies}\\
% %[4]\href{https://www.tiktok.com/creators/creator-portal/en-us/community-guidelines-and-safety/community-guidelines/}{TikTok Community Guidelines}\\
% %[5]\href{https://about.instagram.com/blog/announcements/instagram-community-guidelines-faqs/}{Instagram Community Guidelines}\\
% %[6]\href{https://support.reddithelp.com/hc/en-us/articles/36004307535}{Reddit Help}\\
% %\end{tabular}
% %} \\ \hline
% %\hline
% \end{tabular}%
% }
% \caption{We summarized 6 communities' standards and regulations about content moderation.}
% \label{tab:communityStandards}
% \end{table*}

% \begin{table*}[]
% \centering
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{|l|llllllll|}
% \hline
% Countries & \multicolumn{1}{l|}{Copyright} & \multicolumn{1}{l|}{Value Align} & \multicolumn{1}{l|}{Terrorism} & \multicolumn{1}{l|}{Fact-check} & \multicolumn{1}{l|}{Illegal} & \multicolumn{1}{l|}{Defame} & \multicolumn{1}{l|}{Hate} & Ref \\ \hline
% \hline
% USA & \multicolumn{1}{l|}{\Checkmark} & \multicolumn{1}{l|}{{\XSolidBrush}} & \multicolumn{1}{l|}{\Checkmark} & \multicolumn{1}{l|}{\XSolidBrush} & \multicolumn{1}{l|}{\Checkmark} & \multicolumn{1}{l|}{\Checkmark} & \multicolumn{1}{l|}{\Checkmark} & Communications Decency Act~\cite{Klosek_2021, USPolicy:online} \\ \hline
% Europe Union & \multicolumn{1}{l|}{\Checkmark} & \multicolumn{1}{l|}{\XSolidBrush} & \multicolumn{1}{l|}{\Checkmark} & \multicolumn{1}{l|}{\Checkmark} & \multicolumn{1}{l|}{\Checkmark} & \multicolumn{1}{l|}{\XSolidBrush} & \multicolumn{1}{l|}{\Checkmark} & Digital Services Act~\cite{european2020digital} \\ \hline
% Japan & \multicolumn{1}{l|}{\Checkmark} & \multicolumn{1}{l|}{\Checkmark} & \multicolumn{1}{l|}{\Checkmark} & \multicolumn{1}{l|}{\Checkmark} & \multicolumn{1}{l|}{\Checkmark} & \multicolumn{1}{l|}{\Checkmark} & \multicolumn{1}{l|}{\Checkmark} & Media Moderation Policy~\cite{japanPolicy:online}\\ \hline
% UK & \multicolumn{1}{l|}{\XSolidBrush} & \multicolumn{1}{l|}{\XSolidBrush} & \multicolumn{1}{l|}{\Checkmark} & \multicolumn{1}{l|}{\XSolidBrush} & \multicolumn{1}{l|}{\Checkmark} & \multicolumn{1}{l|}{\XSolidBrush} & \multicolumn{1}{l|}{\Checkmark} & Online Safety Bill Guide~\cite{ukPolicy:online} \\ \hline
% Canada & \multicolumn{1}{l|}{\XSolidBrush} & \multicolumn{1}{l|}{\XSolidBrush} & \multicolumn{1}{l|}{\Checkmark} & \multicolumn{1}{l|}{\XSolidBrush} & \multicolumn{1}{l|}{\Checkmark} & \multicolumn{1}{l|}{\XSolidBrush} & \multicolumn{1}{l|}{\Checkmark} & Canada Law~\cite{CAPolicy:online}\\ \hline
% India & \multicolumn{1}{l|}{\XSolidBrush} & \multicolumn{1}{l|}{\XSolidBrush} & \multicolumn{1}{l|}{\XSolidBrush} & \multicolumn{1}{l|}{\Checkmark} & \multicolumn{1}{l|}{\Checkmark} & \multicolumn{1}{l|}{\Checkmark} & \multicolumn{1}{l|}{\Checkmark} & IT Rules~\cite{IndiaPolicy:online} \\ \hline
% China & \multicolumn{1}{l|}{\Checkmark} & \multicolumn{1}{l|}{\Checkmark} & \multicolumn{1}{l|}{\Checkmark} & \multicolumn{1}{l|}{\Checkmark} & \multicolumn{1}{l|}{\Checkmark} & \multicolumn{1}{l|}{\Checkmark} & \multicolumn{1}{l|}{\Checkmark} & \begin{tabular}[c]{@{}l@{}}Basic requirements for security of generative artificial intelligence services~\cite{CNGenAIPolicy:online}\\ Provisions on Ecological Governance of Network Information Content~\cite{CNPolicy:online}\end{tabular} \\ \hline
% \hline
% \end{tabular}%
% }
% \caption{We summarized current laws and regulations of some countries. To be noted, only China's regulation has AIGC-specific parts until our submission.}
% \label{tab:lawStudy}
% \end{table*}


% \subsubsection{Why Social Platforms Want to Moderate Content?}
% \label{sec:understanding:platform:why}

\subsection{Multiple Policies Moderation}\label{sec:enforce:multi}

\begin{figure}[htb!]
\centering
\includegraphics[width=0.45\textwidth]{figs/Cos_sim.pdf}
\caption{The Cosine Similarity between each pair of concept's task vector in gambling}
\label{fig:cos_sim}
\end{figure}

\begin{figure}[htb!]
\centering
\includegraphics[width=0.45\textwidth]{figs/cosSim_eachLayer.pdf}
\caption{The Cosine Similarity of each layer between 2 task vectors \qiyu{I do not get the meaning of this figure.}}
\label{fig:cos_sim_each}
\end{figure}

\par As the various demands of ethics requirements for stable diffusion, \sysname\ may have requirements to moderate multiple concepts from the stable diffusion model. To combine the multiple concepts moderation, the most natural way is to simply accumulate multiple concepts' task vectors to create a combined task vector (also the way declared in \cite{ilharco2022editing}). However, direct accumulation of task vectors is proven to be not ideal. We use the small concepts' task vectors within the big concept "gambling" to compute each pair's cosine similarity as shown in Fig. \ref{fig:cos_sim}. We can have the same conclusion with \cite{ilharco2022editing} that, most task vectors are nearly orthogonal. However, when we compute each layer's cosine similarity between 2 task vectors, we can observe from Fig. \ref{fig:cos_sim_each} that some layers' parameters between 2 task vectors have high cosine similarity, which means they are not nearly orthogonal. So directly accumulating multiple task vectors is not a good way to moderate multiple concepts in stable diffusion. \cite{ilharco2022editing} mentioned using the adaptive scale to adjust each task vector's weight, it is not a good solution since applying the adaptive scale to each whole task vector will greatly reduce the effect of unorthogonal part of the weight parameter resulting in moderation effect reduction. Thus, we use tie merging from \cite{yadav2023ties-merging} which merges multiple concepts using a selective parameter merging method. \sysname will intelligently choose to directly take value from a single task vector's value or merge multiple task vectors' values on each single parameter.











% \subsection{Summary}
% \par By drawing an analogy between social media platforms and GenAI, we understand the need for content moderation in GenAI, and identify the gap between current GenAI content moderation and social platforms' expectations. We can have the conclusion that current content moderation in GenAI can not meet the need.



%\begin{table*}[]
%\centering
%\resizebox{\textwidth}{!}{%
%\begin{tabular}{|l|l|l|l|l|l|l|l|}
%\hline

%\textbf{Moderation}             & \textbf{Fact-Checking}            & \textbf{Values Align}             & \textbf{Hard to bypass}           & \textbf{Fine-grained Control}     & \textbf{Automatically}            & \textbf{Protect Reviewer}         & \textbf{Fairness}                 \\ \hline

%Human Detection                 & {\color[HTML]{00B050} \Checkmark} & {\color[HTML]{00B050} \Checkmark} & {\color[HTML]{00B050} \Checkmark} & {\color[HTML]{00B050} \Checkmark} & {\color[HTML]{FF0000} \textbf{\XSolidBrush}} & {\color[HTML]{FF0000} \textbf{\XSolidBrush}} & {\color[HTML]{FF0000} \textbf{\XSolidBrush}} \\ \hline

%AI Detection                    & {\color[HTML]{FF0000} \textbf{\XSolidBrush}} & {\color[HTML]{FF0000} \textbf{\XSolidBrush}} & {\color[HTML]{FF0000} \textbf{\XSolidBrush}} & {\color[HTML]{FF0000} \textbf{\XSolidBrush}} & {\color[HTML]{00B050} \Checkmark} & {\color[HTML]{00B050} \Checkmark} & {\color[HTML]{FFC000} \textbf{$\circ$}} \\ \hline

%Hybrid Detection                & {\color[HTML]{FF0000} \textbf{\XSolidBrush}} & {\color[HTML]{FF0000} \textbf{\XSolidBrush}} & {\color[HTML]{FF0000} \textbf{\XSolidBrush}} & {\color[HTML]{FF0000} \textbf{\XSolidBrush}} & {\color[HTML]{FFC000} \textbf{$\circ$}} & {\color[HTML]{FFC000} \textbf{$\circ$}} & {\color[HTML]{FFC000} \textbf{$\circ$}} \\ \hline

%Moderate Prompt                 & {\color[HTML]{FF0000} \textbf{\XSolidBrush}} & {\color[HTML]{FF0000} \textbf{\XSolidBrush}} & {\color[HTML]{FF0000} \textbf{\XSolidBrush}} & {\color[HTML]{FF0000} \textbf{\XSolidBrush}} & {\color[HTML]{00B050} \Checkmark} & {\color[HTML]{00B050} \Checkmark} & {\color[HTML]{00B050} \Checkmark} \\ \hline

%Moderate Generated Images(NSFW) & {\color[HTML]{FF0000} \textbf{\XSolidBrush}} & {\color[HTML]{FF0000} \textbf{\XSolidBrush}} & {\color[HTML]{FF0000} \textbf{\XSolidBrush}} & {\color[HTML]{FF0000} \textbf{\XSolidBrush}} & {\color[HTML]{00B050} \Checkmark} & {\color[HTML]{00B050} \Checkmark} & {\color[HTML]{00B050} \Checkmark} \\ \hline

%Moderate Model Weight           & {\color[HTML]{FF0000} \textbf{\XSolidBrush}} & {\color[HTML]{FF0000} \textbf{\XSolidBrush}} & {\color[HTML]{00B050} \Checkmark} & {\color[HTML]{FF0000} \textbf{\XSolidBrush}} & {\color[HTML]{00B050} \Checkmark} & {\color[HTML]{00B050} \Checkmark} & {\color[HTML]{FFC000} \textbf{$\circ$}} \\ \hline
%\end{tabular}%
%}
%\caption{Summary of current moderation techniques on TTI AIGC model.}
%\label{tab:comparison}
%\end{table*}


% -  draw an analogy between social platform and GenAI => explore content moderation in social platforms
%  method: review community guidelines, literature
%  results: identify 14 common content moderation types

% - the administrators may have different needs of regulation
%     - different content moderation standard on different platforms
%     - different regions will have different laws and regulations for content moderation.
%     - the regulations will also vary with time changes, and new needs may come up with new public opinion events. 

% - GenAI brings more uncertainty to content moderation 
%     - To understand this, we collected and analyzed 153 prompts that may generate different harmful content. In analyzing these prompts and examining the reasons for moderating these contents, we devise a policy formulation to moderate this content
%     - various harm contents caused by the GenAI / complex moderation problems => no one for all policies to govern all the content
%     - different moderation problems can be moderated at different granularity level
%     - can be moderated with different moderation methods
%       four levels (advantage: indexable). 
%             + (noun) remove one specific type of content. e.g., copyright, trademark (selling counterfeit products), etc. 
%             + (adjective) mediate the extent (e.g., too bloody)
%             + (verb) relational behaviors. 
%             + (context). (e.g., no pee in front of Jesus in church) 

% can still infer the content
% results insights: 1. open-vocabulary 2. fine-grained moderation 3. 

% Example prompt candidate list:
% 1. A girl holding a Mickey Mouse doll - Piracy - level 1
% 2. A vegetarian / monk feasts on beef - Social relation harm - level 3 (*Refine)
% 3. Asian squints his eyes - Social relation harm - level 3
% 4. Xenomorph feeding on crewman in sci-fi hallway - Personal emotional harm - level 1/3
% 5. Adam and Eve holding their baby, baby smoking cigarette - Bad behavior spread harm / children harm - level 3
% 6. A mouth full of bacteria. rotten image. realistic photograph - Personal emotional harm - level 2
% 7?. A perfect hand drawn picture of Donald Trump being put into hand cuffs by FBI agents outside of his Florida country club, insanely detailed - Personal relation harm - level 3/4



\subsection{Security Study: Can users attack the moderated models?}
\label{sec:eval:security}

\begin{table*}[]\normalsize
\centering
%\resizebox{\textwidth}{!}{%
\begin{tabular}{p{3cm}|p{0.7cm}|p{0.7cm}|p{0.7cm}|p{0.7cm}|p{0.7cm}|p{0.7cm}|p{0.7cm}|p{0.7cm}|p{0.7cm}|p{0.7cm}|p{0.7cm}|p{0.7cm}}
\hline

\textit{\textbf{Participant}} & E1 & E2 & E3 & E4 & E5 & E6 & E7 & U1 & U2 & U3 & U4 & U5 \\ \hline \hline

\textit{\textbf{Individual Attack No.}} & Failed & 67 & Failed & Failed & 32 & 41 & Failed & Failed & Failed & Failed & Failed & Failed\\ \hline

\textit{\textbf{Knowledgable Attack No.}} & Failed & 5 & Failed & Failed & 11 & 21 & Failed & Failed & 67 & 23 & 12 & Failed \\ \hline
\end{tabular}
%}
\caption{We asked participants to try to bypass the moderation policy in 100 prompts in the first phase. We noted the number of attempts until a successful attack in the first phase as \textit{\textbf{Individual Attack Number}} (each participant attacks the moderated model individually). Then we grouped all the participants to share their successful bypass experience with each other. After that, we asked the participants to bypass the moderation policy again in 100 prompts in the second phase. We noted We noted the number of attempts until a successful attack in the second phase as \textit{\textbf{Knowledgable Attack Number}}.}
\label{tab:eval:atkStudy}
\end{table*}

\par Subsequently, we engaged participants in an exercise aimed at attacking the robustness of the moderated model. The objective was to bypass the moderation policy, thereby prompting the Text-to-Image (TTI) model to produce content that was originally deemed harmful. This exercise was structured into two distinct phases:

\begin{itemize}
    \item \textbf{First Phase (Individual Attack)}: Participants selected a specific moderation policy to target. Each was given 100 attempts to input varying prompts into the moderated model. Successful bypassing of the moderation policy was recorded as ``1st Phase Atk. No.'' in Table \ref{tab:eval:atkStudy}. Conversely, if a participant failed to breach the policy within these attempts, this outcome was noted as ``Failed'' in the same table.
    \item \textbf{Second Phase (Knowledgable Attack)}: Following the initial phase, we held a workshop to share the successful bypass strategies and encouraged participants to collaborate in brainstorming and identifying potential methods for circumvention. Subsequently, they were given another set of 100 prompt attempts to challenge the moderation mechanisms of the models.
\end{itemize}





\sssec{Checking Conflicts between Policies}
\par In scenarios where \sysname\ must integrate multiple moderation policies, conflicts can arise between two distinct policies. For instance, simultaneously applying policies like \textbf{``Blocking'' Mickey Mouse} and \textbf{``Removing'' Mickey Mouse} would lead to a conflict, as these two actions inherently contradict each other. To address such conflicts, we have developed specific heuristics within \sysname:

\par First, we identified five relations between two contents (noted as content $\alpha$ and $\beta$) as $rel(\alpha, \beta)$:
\begin{itemize}
    \item \textbf{Belong ($\alpha\subseteq\beta$)}: Content $\alpha$ belongs to content $\beta$, for instance, ``Mickey Mouse'' belongs to ``Disneyland''.
    \item \textbf{Include ($\alpha\supseteq\beta$)}: Content $\alpha$ includes content $\beta$, for instance, ``Disneyland'' includes ``Mickey Mouse''.
    \item \textbf{Equal ($\alpha=\beta$)}: Content $\alpha$ and content $\beta$ are the same.
    \item \textbf{Juxtapose ($\alpha\oslash\beta$)}: Content $\alpha$ and content $\beta$ has no relation with each other, for instance, ``Blood'' and ``Flower''.
    \item \textbf{Intersect ($\alpha\cap\beta$)}: Content $\alpha$ and content $\beta$ have intersection with each other, for instance, ``Animal'' and ``Disneyland'' have intersected content ``Mickey Mouse''.
\end{itemize}

Then for $rel(\alpha, \beta)$, \sysname will call LLM to judge the relationship between $\alpha$ and $\beta$ using the prompt template in Appendix Prompt. \ref{prompt:contentRelation}, and return the value within the five identified relations.

\par The resolution process begins by parsing two policies to the combination of a series of task vectors. Then \sysname\ will examine conflicts between two task vectors. We have established a set of heuristics to manage and reconcile every possible pair of conflicting task vectors. These heuristics are systematically detailed in Table. \ref{tab:conflicts}, providing a structured approach to resolving policy conflicts within the system. If any two task vectors conflict with each other, the two policies conflict. This ensures that \sysname can effectively handle multiple, potentially conflicting moderation policies without compromising its overall functionality and efficiency. 


\begin{table*}[]
\centering
\begin{tabular}{M{3cm}|M{1cm}M{1cm}M{1cm}M{1cm}M{1cm}|M{1cm}M{1cm}M{1cm}M{1cm}M{1cm}}
\hline
& \multicolumn{5}{l}{$T_{x_1\to y_1}+T_{x_2\to y_2}$} & \multicolumn{5}{l}{$T_{x_1\to y_1}-T_{x_2\to y_2}$} \\ \hline\hline
$rel(x_1, x_2)$/$rel(y_1, y_2)$ & $\subseteq$ & $\supseteq$ & $=$ & $\oslash$ & $\cap$ & $\subseteq$ & $\supseteq$ & $=$ & $\oslash$ & $\cap$ \\ \hline
$\subseteq$ & \Checkmark & \Checkmark & \Checkmark & \Checkmark & \Checkmark & \Checkmark & \Checkmark & \Checkmark & \Checkmark & \Checkmark \\ \hline
$\supseteq$ & \XSolidBrush & \XSolidBrush & \XSolidBrush & \XSolidBrush & \XSolidBrush & \XSolidBrush & \XSolidBrush & \Checkmark & \XSolidBrush & \XSolidBrush \\ \hline
$=$ & \XSolidBrush & \XSolidBrush & \XSolidBrush & \XSolidBrush & \XSolidBrush & \Checkmark & \XSolidBrush & \XSolidBrush & \Checkmark & \Checkmark \\ \hline
$\oslash$ & \XSolidBrush & \XSolidBrush & \XSolidBrush & \XSolidBrush & \XSolidBrush & \Checkmark & \Checkmark & \Checkmark & \Checkmark & \Checkmark \\ \hline
$\cap$ & \XSolidBrush & \XSolidBrush & \XSolidBrush & \XSolidBrush & \XSolidBrush & \XSolidBrush & \XSolidBrush & \XSolidBrush & \XSolidBrush & \XSolidBrush \\\hline\hline
\end{tabular}%
\caption{The table for judging task vector conflicts. \Checkmark denotes there is no conflict, while \XSolidBrush means conflict.}
\label{tab:conflicts}
\end{table*}

\begin{table*}[]
\centering
%\resizebox{\textwidth}{!}{%
\begin{tabular}{m{1.2cm}p{1.4cm}p{2.5cm}p{5cm}p{2cm}p{2cm}}%{lllllll}
\hline
Element & Method & Purpose  & Moderation Policy & Example Input & Example \par Output \\ \hline 

\hline
Object & Replacing object & 
\raisebox{-.5\height}{\begin{minipage}[b]{2.5cm}
- Copyright 
\end{minipage}}
%& 
%\raisebox{-.5\height}{\begin{minipage}[b]{3.5cm}
%1girl, holding a Mickey Mouse doll, beautiful detailed eyes, beautiful detailed lips, extremely detailed eyes and face, long eyelashes, cute girl, smiling girl, detailed clothes, colorful background, playful expression, vivid colors, realistic lighting, portrait, ultra-detailed, highres, masterpiece:1.2 
%\end{minipage}}
& 
\raisebox{-.5\height}{\begin{minipage}[b]{5cm} 
\vspace{0pt}
Content:
\par \hspace{0.2cm}\levelAword:\levelA{``Mickey Mouse"}
\par \hspace{0.2cm}\hspace{0.5cm}$\Rightarrow$\levelA{``Mouse"}
%\par Purpose=\textcolor{brown}{``Copyright"},
%\par Method=\textcolor{brown}{``Replace"}

\end{minipage}}
& \begin{minipage}[b]{2cm} \raisebox{-.5\height}{\includegraphics[width=\linewidth]{figs/examples/1_mickey_mouse_before.png}}\end{minipage} 
& \begin{minipage}[b]{2cm}\centering \raisebox{-.5\height}{\includegraphics[width=\linewidth]{figs/examples/mickeyMouse-after.png}}\end{minipage} \\ \hline
Style & Mitigate style & 
\raisebox{-.5\height}{\begin{minipage}[b]{2.5cm}
- Horror
\\- Gore
\\- Violence 
\end{minipage}}
%& 
%\raisebox{-.5\height}{\begin{minipage}[b]{3.5cm}
%realistic style, photo of a soldier, writhing in pain, falling into the ground, bloody wires bursting out of his body, expression of agony, military uniform, detailed facial features, intense emotion, overcast sky, shadows cast by the soldier, focus on the soldier's pain and the wires.
%\end{minipage}}
& 
\raisebox{-.5\height}{\begin{minipage}[b]{5cm} 

Content:
\par \hspace{0.2cm}\levelBword:\levelB{``Bloody"}
%\par Purpose=\textcolor{brown}{``Horror"},
%\par Method=\textcolor{brown}{``Mitigate"}

\end{minipage}}
& 
\begin{minipage}[b]{2cm}\centering \raisebox{-.5\height}{\includegraphics[width=\linewidth]{figs/examples/bloodSoldier-before.png}}\end{minipage} 
& 
\begin{minipage}[b]{2cm}\centering \raisebox{-.5\height}{\includegraphics[width=\linewidth]{figs/examples/bloodSoldier-after.png}}\end{minipage} \\ \hline

Action & Removing \levelCword &
\raisebox{-.5\height}{\begin{minipage}[b]{2.5cm}
- Children Harm
\end{minipage}}
%& 
%\raisebox{-.5\height}{\begin{minipage}[b]{3.5cm}
%A woman sitting on the sofa with sunken eyes, wrinkles, dark hair, holding a pipe in her hands and smoking marijuana, real style, high res, gray tones
%\end{minipage}}
& 
\raisebox{-.5\height}{\begin{minipage}[b]{5cm} 

Content:
\par \hspace{0.2cm}\levelCword:\levelC{``smoking marijuana"}
%\par Purpose=\textcolor{brown}{``Illegal Activities"},
%\par Method=\textcolor{brown}{``Removing"}

\end{minipage}}
& \begin{minipage}[b]{2cm}\centering \raisebox{-.5\height}{\includegraphics[width=\linewidth]{figs/examples/drug-before.png}}\end{minipage} 
& \begin{minipage}[b]{2cm}\centering \raisebox{-.5\height}{\includegraphics[width=\linewidth]{figs/examples/drug-after.png}}\end{minipage} \\ \hline

Combined & Replacing \levelCword & 
\raisebox{-.5\height}{\begin{minipage}[b]{2.5cm}
- Violence
\\- Illegal Activities
\\- Disinformation
\\- Defamation
%\\- Political Propaganda 
\end{minipage}}
%& 
%\raisebox{-.5\height}{\begin{minipage}[b]{3.5cm}
%hyper-realistic photo of a fight between Donald Trump and a New York City police officers, detailed trump face, realistic police figure, New York street scene 
%\end{minipage}}
& 
\raisebox{-.5\height}{\begin{minipage}[b]{5cm} 

Content:
\par \hspace{0.2cm}\levelAword:\levelA{``Trump"}
\par \hspace{0.2cm}\levelCword:\levelC{``Fight with police officers"} 
\par \hspace{0.2cm}\hspace{0.5cm}$\Rightarrow$\levelC{``Stand with police officers"}
%\par \hspace{1cm} $\Downarrow $
%\par replaced\_content:
%\par \hspace{0.2cm}\levelAword:\levelA{``Trump"}
%\par \hspace{0.2cm}\levelCword:\levelC{``Stand"}
%\par Purpose=\textcolor{brown}{``Defamation"},
%\par Method=\textcolor{brown}{``Replace"}

\end{minipage}}
& \begin{minipage}[b]{2cm}\centering \raisebox{-.5\height}{\includegraphics[width=\linewidth]{figs/examples/trumpNYPolice-before.png}}\end{minipage} 
& \begin{minipage}[b]{2cm}\centering \raisebox{-.5\height}{\includegraphics[width=\linewidth]{figs/examples/trumpNYPolice-after.png}}\end{minipage} \\ \hline
\end{tabular}%
%}
\caption{Four example policies for content moderation in Stable Diffusion. \haojian{The text style of the policy language is not consistent. Capital case, font, symbols. Smoking marijuana is not an illegal activity. Consider to make all text top aligned.}}
\label{tab:exampleShow}
\end{table*}

\sssec{Content Moderation} 

Content moderation has received a large focus both in security and human-computer interaction fields. Harmful content can result in various bad effects, such as spreading fake news \cite{hjorth2019ideological} and manipulating political elections \cite{dutt2019senator}. To define what content needs to be moderation, \cite{scheuerman2021framework} provides the detailed category of harm of content, and summarizes severity metrics. Previous research of content moderation mainly focuses on moderating harmful content on social platforms. Social platforms themselves provide various content moderation techniques. Facebook/Meta, Twitter, etc. rely on the employment of some specialists who are paid to manually moderate content \cite{chen2014laborers, roberts2016commercial}, however other platforms, such as Reddit \cite{jhaver2019human, matias2016civic} recruit some volunteers as content moderators to keep the community environment healthy by themselves. However, manual moderation brings high costs which are hard to accept for social platforms. Platforms also apply \textbf{rule-based detection} to automatically moderate content. Platforms have developed a series of algorithm-based detection systems to automatically detect toxic images in users' published contents \cite{niu2008overview}. Some AI-based detection systems have also been invented to moderate content [].

\par With the avenue of TTI AIGC, content moderation has been broadly changed. In traditional content moderation, moderators are only allowed to moderate the content already produced by the publishers. However, the emergence of TTI AIGC brings moderators with the ability to directly moderate content publishers' production tools, which means the TTI AIGC models here. To provide content moderation, previous researchers have designed several approaches. The negative prompt is designed to moderate the prompts before the prompts are input into the TTI models \cite{schramowski2023safe}. However, it is easy to bypass such moderation using adversarial examples \cite{yang2023sneakyprompt}. Different from moderating prompts, \cite{gandikota2023erasing} provides a way to directly method to moderate the model weight to erase the model's ability to generate harmful content, however, such approaches bring more system overhead than moderating prompts. 

\par However, there has not been a systematic study of content moderation in TTI AIGC. Previous researchers do not provide a full study about what to moderate and how to moderate in TTI AIGC.

%\subsection{Ethical Generative AI}
%Since the explode of the generative AI in recent months, the ethics of generative AI has catched many researchers' attention. Pretrained generative AI models are prone to generating racist, sexist, or otherwise toxic language which hinders their safe deployment. 
%Gehman et al. \cite{gehman2020realtoxicityprompts} have investigated the extent to which pretrained LMs can be prompted to generate toxic language, and the effectiveness of controllable text generation algorithms at preventing such toxic degeneration. They create and release a dataset to find the toxic degeneration of pretrained LMs. % evaluate toxic in LLMs
%Deshpande et al. \cite{deshpande2023toxicity} systematically evaluate the toxicity of ChatGPT. They showed that the generation of ChatGPT within a given persona will lead to the significant increase of toxic content. % evaluate toxic in LLMs
%Wallace et al. \cite{wallace2019universal} show the toxicity of LLMs by adding a `trigger' to guide the LLM to produce toxic content. % evaluate toxic in LLMs
%Wang et al. \cite{wang2022exploring} explore domain-adaptive training to reduce the toxicity of language models and propose to leverage the generative power of LMs and generate nontoxic datasets for domain-adaptive training to mitigate toxicity. % mitigate toxic in LLMs
%Ousidhoum et al. \cite{ousidhoum2021probing} propose a method based on logistic regression classifiers to probe English, French, and Arabic PTLMs and quantify the potentially harmful content that they convey with respect to a set of templates. % mitigate toxic in LLMs



% The service proprietor maintains full control over their machines, ensuring that no malicious software was on the system.

% In doing so, the service provider can restrict potential misuse by users.
% , 

% \peiran{We focus on the scenario where the user does not fine-tune the stable diffusion model locally, but only accesses the inference function of the stable diffusion model through the online platform API, or only downloads the model creation image provided by the online platform. In this scenario, three types of potential malicious users are considered in our threat model: 1) curious teenagers; 2) malicious users who try to induce the model to generate harmful content to attack the model publisher; 3) malicious authors who exploit the model for malicious content creation. Curious teenagers may use models to generate harmful content that endangers their healthy growth, while some other malicious users deliberately try to let models generate harmful content. The generated harmful content will be used as evidence to accuse model publishers of violating relevant regulations. At the same time, Some malicious creators want to use models for the creation of malicious content. Further, to comply with regional regulations and prevent the above three categories of users from using the model to generate harmful content, market administrators will need to implement additional layers of moderation, similar to how today's social media platforms modem user posts~\cite{singhal2023sok}. Depending on regional regulations, users can download a modified version of the model instead of the original pretrained model. Modified versions of the model will be customized according to platform and regional regulations, preventing teens and other users from using the GenAI model to draw harmful content prohibited by specific policies.}

% \begin{CJK}{UTF8}{gbsn}
% \par \peiran{我们关注用户不在本地微调稳定扩散模型，而仅通过在线平台 API 访问稳定扩散模型的推理功能、或者仅下载线上平台提供的模型创建图像的场景。 在这种场景下，我们的威胁模型中考虑三类用户：1）好奇的青少年；2）尝试诱导模型生成有害内容来攻击模型发布者的恶意用户；3）利用模型进行恶意内容创作的恶意创作者。 好奇的青少年可能会使用模型生成有害的内容危害其的健康成长，而另外一些恶意用户故意尝试让模型生成有害内容，生成的有害内容将被利用作为证据指控模型发布者违反相关法规，同时还有一些恶意创作者想要使用模型进行恶意内容的创作。进一步的，为了符合地区法规并且防止以上三类用户使用模型生成有害内容，市场管理员将需要实施额外的审核层，类似于当今社交媒体平台审核用户帖子的方式~\cite{singhal2023sok}。 根据地区规定，用户可以下载模型的修改版本，而不是原始的预训练模型。 该模型的修改版本将根据平台规定和地区规定进行定制，从而防止青少年和其他用户使用GenAI模型绘制特定政策禁止的有害内容。}
% \end{CJK}

% \par \peiran{We designed a new system \sysname to conduct text-to-image model moderation. A major challenge in this design is figuring out what is harmful and in what form the model should be moderately controlled. First, the open vocabulary nature of content moderation is extremely complex and diverse. In addition, the existing content moderation methods of the text-to-image model are too rough and cannot meet the fine-grained content moderation. The weight space of text-to-image graph models is vast and diverse, making it difficult to adjust content in text-to-image models. Existing content moderation methods for text-to-image models (negative prompts, model editing, NSFW filters) are easily bypassed and have high false positive and false negative rates.}

% \begin{CJK}{UTF8}{gbsn}
% \par \peiran{我们设计了一个新的系统\sysname来进行AIGC模型的审核。此设计中的一个主要挑战是弄清楚哪些有害内容，以及应以何种形式对模型进行适度控制。 首先，内容审核的开放词汇性质极其复杂多样。 此外，现有的文生图模型的内容审核方法过于粗糙，无法满足细粒度的内容审核。文生图模型的权重空间广阔且多样，使得文本到图像模型中的内容难以调节。 现有的文生图模型的内容审核方法（否定提示、模型编辑、NSFW 过滤器）很容易被绕过，存在较高的误报率和漏报率。}
% \end{CJK}

% \par\peiran{\sysname\ first applies an element-based policy primitive to represent the moderated content. This primitive parsed the natural language policy into a three-element structure to provide fine-grained moderation control. To solve the open vocabulary problem, an element-wise content expansion is applied to expand the single content of user-authored policy into an open vocabulary prompts dataset. After that, we apply a model weight reverse fine-tuning process using the expanded dataset to eliminate the model knowledge of the moderated content from the Stable Diffusion model. \sysname\ also provides three different moderation methods for administrators to craft diverse moderation policies.}
% \begin{CJK}{UTF8}{gbsn}
% \par \peiran{\sysname\ 首先应用基于元素的策略原语来表示审核策略的内容。 该原语将自然语言策略解析为包含object、style和action的三元素结构，提供细粒度的审核控制。进一步的，为了解决开放词汇问题，\sysname\ 基于三元素结构，使用LLM对审核策略的内容进行了query expansion，将用户编写的策略中的单一内容扩展为开放词汇提示数据集。 之后，\sysname\ 使用该数据集进行模型权重反向微调过程，消除模型中需要被审核内容的模型知识，使模型失去生成被审核内容的能力。\sysname\ 还提供了三种不同的审核方法，供管理员制定多样的审核效果选择。}
% \end{CJK}


% potential harmful content produced by GenAI services
% Then we analyzed what difference the era of GenAI brings to content moderation. We first summarized what harm is brought by the misuse of GenAI to the world. Then we explored different online GenAI platforms to explore whether they provide good content policies and strong content moderation or not. At last, we provided a category of potentially harmful content that may be generated by GenAI via card sorting.

% \subsubsection{Harm Brought by the Misuse of GenAI}
% \label{sec:understanding:GenAI:harm}




% \par First of all, the abuse of Stable Diffusion has already created certain harmful events:
% \par \textbf{The GenAI model can be used to generate bloody and violent images to create emotional harm.} Though NSFW filters have been applied in many online GenAI model platforms to provide content filtering against horrible and bloody images, people can still bypass such NSFW filters or just deploy the model locally to disable it. \cite{lost2022make} has shown several cases to generate bloody and violent images. Such images may be very harmful if the users are children, elders, or some other populations who are vulnerable to it, it will create huge emotional damage to them.
% \par \textbf{People can use the GenAI model to create discrimination images.} The fairness problems have been discussed a lot of times since the bias persists in the weight of the deep learning model. It is also a problem in GenAI models. The world according to Stable Diffusion is run by White male CEOs. Women are rarely doctors, lawyers, or judges. Men with dark skin commit crimes, while women with dark skin flip burgers \cite{leonardo2023humans}. Researchers analyze the stereotype of the Stable Diffusion model. They find that the Stable Diffusion model corresponds to a career with ethnicity and gender. Furthermore, when asking the model to draw the faces of criminals, it shows even greater discrimination in skin color and ethnicity.
% \par \textbf{GenAI model can be used to create illegal child sexual images.} Paedophiles are using artificial intelligence (AI) technology to create and sell life-like child sexual abuse material \cite{angus2023illegal}. Some are accessing the images by paying subscriptions to accounts on mainstream content-sharing sites such as Patreon. A man in South Korea was sentenced in September to 2.5 years in prison for using artificial intelligence to create 360 virtual child abuse images \cite{matt2023AI}. 
% \par \textbf{The GenAI model can also be utilized to bully and harass}. In some cases, kids are using these tools on each other to bully and harass. At a school in southwestern Spain, police have been investigating teens’ alleged use of a phone app to make their fully dressed schoolmates appear nude in photos \cite{matt2023AI}.
% \par \textbf{The inherent copyright problem of the GenAI model has also been discussed a lot of times.} Stable Diffusion has been law-suited many times since the generated images contain certain artists' masterpieces and styles \cite{matthew2023we}. Moreover, it happens that when the model draws the logo `Getty Image' of image image-sharing website. Furthermore, the copyright of celebrity can be invaded as well. Tom Hanks has issued a warning after an AI-generated version of the actor was used to promote a dental plan.
% \par \textbf{The misuse of GenAI models can create a huge social impact in the real world.} The world’s most popular text-to-image generators – Midjourney, DALL-E 2, and Stable Diffusion – accepted on average over 85\% of prompts that sought to generate fake political news, according to a new report \cite{ben2023AI}. Fake political images have been shown to have a large power in affecting the real world's politics. Researchers have tested the reality of generated Fake News images of different models. All in all, their images still don't compare to real photos. However, they remain effective against disinformation campaigns, such as the alleged Pentagon bombing in May, which briefly sent the stock market tumbling. In Paris, a popular Twitter user posted three photos of French President Emmanuel Macron sprinting between riot police and protesters, surrounded by billows of smoke. The images, which have been viewed more than 30,000 times, are fake. But that’s not so obvious to anyone who doesn’t follow the growth of artificial intelligence image generators \cite{parmy2023commentary}. The GenAI has also been used in creating fake political images to influence the election: US presidential candidate and Florida Governor Ron DeSantis is trying to undermine Trump's 2024 presidential campaign by releasing an image that features Donald Trump hugging Dr. Anthony Fauci (and this image is proven to be AI-generated later).

% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \begin{table*}[]
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{|p{4cm}|p{2cm}|p{2cm}|p{2cm}|p{2cm}|p{2cm}|p{2cm}|p{2cm}|p{2cm}|p{2cm}|}
% \hline
% Platform                 & Dream Studio & Playground & GetImg.AI     & leonardo.ai & dezgo & Lexica        & Picso & Holara & Stablebility.AI \\ \hline
% \hline
% Content Policy           & Well         & Well          & Vague         & Vague       & Vague & No            & Vague & Vague  & Vague           \\ \hline
% Strong Content Moderation  & \XSolidBrush            & \XSolidBrush             & \XSolidBrush             & \XSolidBrush           & \XSolidBrush     & \XSolidBrush             & \XSolidBrush     & \XSolidBrush      & \XSolidBrush               \\ \hline
% Content Responsibility   & User         & No Mention & No Mention & User        & User  & No Mention & User  & User   & User            \\ \hline
% Misinformation           & \Checkmark            & \Checkmark             & \Checkmark             & \Checkmark           & \XSolidBrush     & \XSolidBrush             & \Checkmark     & \XSolidBrush      & \Checkmark               \\ \hline
% Violence                 & \Checkmark            & \Checkmark             & \Checkmark             & \Checkmark           & \Checkmark     & \XSolidBrush             & \XSolidBrush     & \XSolidBrush      & \Checkmark               \\ \hline
% Violent Content          & \Checkmark            & \Checkmark             & \XSolidBrush             & \Checkmark           & \Checkmark     & \XSolidBrush             & \XSolidBrush     & \XSolidBrush      & \Checkmark               \\ \hline
% Hate Behavior            & \Checkmark            & \Checkmark             & \Checkmark             & \Checkmark           & \XSolidBrush     & \XSolidBrush             & \Checkmark     & \XSolidBrush      & \Checkmark               \\ \hline
% Bully \& Harrass         & \Checkmark            & \Checkmark             & \Checkmark             & \Checkmark           & \XSolidBrush     & \XSolidBrush             & \Checkmark     & \XSolidBrush      & \Checkmark               \\ \hline
% Adult Nudity             & \Checkmark            & \Checkmark             & \XSolidBrush             & \Checkmark           & \XSolidBrush     & \XSolidBrush             & \Checkmark     & \XSolidBrush      & \XSolidBrush               \\ \hline
% Illegal Items \& Service & \Checkmark            & \Checkmark             & \XSolidBrush             & \Checkmark           & \Checkmark     & \XSolidBrush             & \Checkmark     & \Checkmark      & \Checkmark               \\ \hline
% Abuse \& Explotiation    & \Checkmark            & \XSolidBrush             & \XSolidBrush             & \Checkmark           & \XSolidBrush     & \XSolidBrush             & \XSolidBrush     & \XSolidBrush      & \Checkmark               \\ \hline
% Self-Harm                & \Checkmark            & \Checkmark             & \XSolidBrush             & \XSolidBrush           & \XSolidBrush     & \XSolidBrush             & \XSolidBrush     & \XSolidBrush      & \XSolidBrush               \\ \hline
% Child Sex\&Abuse         & \Checkmark            & \Checkmark             & \Checkmark             & \Checkmark           & \Checkmark     & \XSolidBrush             & \XSolidBrush     & \XSolidBrush      & \Checkmark               \\ \hline
% Graphic Content          & \Checkmark            & \XSolidBrush             & \XSolidBrush             & \XSolidBrush           & \XSolidBrush     & \XSolidBrush             & \Checkmark     & \XSolidBrush      & \XSolidBrush               \\ \hline
% Copyright                & \Checkmark            & \Checkmark             & \Checkmark             & \Checkmark           & \Checkmark     & \Checkmark             & \Checkmark     & \Checkmark      & \Checkmark               \\ \hline
% Personal Privacy         & \Checkmark            & \XSolidBrush             & \XSolidBrush             & \Checkmark           & \Checkmark     & \XSolidBrush             & \Checkmark     & \XSolidBrush      & \XSolidBrush               \\ \hline
% Weapon Content           & \XSolidBrush            & \XSolidBrush             & \XSolidBrush             & \XSolidBrush           & \XSolidBrush     & \XSolidBrush             & \XSolidBrush     & \XSolidBrush      & \XSolidBrush               \\ \hline\hline
% \end{tabular}%
% }
% \caption{Summarize 9 popular GenAI online platforms. Most of them provide a content policy but not well documented. And none of them provide strong content moderation aligning with their content policies.}
% \label{tab:genAIPolicy}
% \end{table*}
% \subsubsection{Summarize GenAI Platforms' Content Policies}
% \label{sec:understanding:GenAI:policy}

% \par Then we collected content moderation policies from 9 popular online GenAI platforms in Table \ref{tab:genAIPolicy}.
% \par \textbf{Most of them provide content policies, but their policies are very vague.} Only 2 platforms provide well-documented statements of content policies. Furthermore, most policies do not cover the moderated items provided by social platforms as shown in Table. \ref{tab:communityStandards}. This indicates that the content policies of most online GenAI platforms are not enough to tackle the content moderation required by social platforms.
%\par \textbf{The platforms do not provide strong content moderation.} Furthermore, to see if the platform moderates the content it stated in its content policy or not, we explore each platform's performance. The results show that none of the platforms achieve full content moderation regulated by their own content policies. All of them only have the ability to deal with nudity content.

% \subsubsection{What Harmful Content GenAI may Produce}
% \label{sec:understanding:GenAI:what}
% \par Based upon previous analysis about social platform regulations and harm brought by the misuse of GenAI, we made a card-sorting process to figure out what content needed to be moderated in the era of GenAI to understand the content that needed to be moderated in GenAI.

%Second, \textbf{the open-vocabulary nature of prompts} presents a significant challenge in moderating AI-generated content. It allows prompts to encompass arbitrary concepts and thereby derive a vast and diverse range of possible content outputs, making it difficult to establish comprehensive moderation criteria. It also introduces semantic ambiguity that each concept can take a different form, making it difficult to comprehensively cover all cases that require moderation. 

% Second, \textbf{the open-vocabulary nature of prompts} presents a significant challenge in content moderation within image-to-text service. This feature allows prompts to encompass a wide range of concepts, leading to a diverse array of potential content outputs. Not only does this make establishing comprehensive moderation criteria complex, but it also introduces semantic ambiguity, as each concept can manifest in various forms. For instance, models like Stable Diffusion can generate images based on any textual prompt provided by users, making it exceedingly difficult to predict and moderate all possible outputs.  The open-vocabulary nature of these prompts means that moderation systems must be capable of handling an extremely broad spectrum of concepts and themes.

% In this context, content moderation must consider not just the visual content of the images but also understand and interpret the underlying meanings and contexts of user prompts.

% while also being able to identify and address prompts that could lead to the generation of inappropriate or harmful content. 

% Moreover, given the capability of these AI models (like Stable Diffusion) to produce highly realistic images, their potential to create misleading or harmful visual content further complicates the moderation task. Therefore, developing effective content moderation strategies and tools to address the challenges posed by open-vocabulary-prompted AI-generated content becomes an urgent and complex task.

% \sssec{Harmful Content Definition in Stable Diffusion}
% Drawing from our previously gathered harmful prompt examples, we now explore how a harmful content is characterized by the prompt produced by a text-to-image model. At first, we identify the primary elements of a stable diffusion prompt as follows:
% \begin{itemize}
% \item \textbf{Subject Description}: This necessitates a clear depiction of the principal subject intended for visualization in the image. This subject may encompass an object, a scene, an activity, or a conceptual idea.
% \item \textbf{Style and Mood}: This involves specifying the desired artistic style (e.g., realism, impressionism, surrealism, etc.), along with the overall emotional tone or atmosphere (such as mystery, joy, serenity, etc.).
%\item \textbf{Details and Features}: This entails incorporating specific details or characteristics, which can include unique objects, characters, or elements of the background.

% \par The prompt in a text-to-image (TTI) model can be regarded as the content definition within the model. Building upon our analysis of the components of a stable diffusion prompt, we now begin with the card sorting examples to address the concept of harmful content in stable diffusion. This exploration involves examining the types of content that may be considered damaging or inappropriate within the context of the generated images and their potential impact.

% \par First of all, the most directly damaging content could be illegal or detrimental objects, such as horrific creatures or items related to piracy, as defined in the ``\textbf{Subject Description}'' of a Stable Diffusion prompt. We categorize such detrimental content under ``\textit{\levelAword}''.

% \par Additionally, harmful content might encompass certain styles detailed in the ``\textbf{Style and Mood}'' section, like gore, blood, or various dark themes, potentially causing emotional distress. This category encapsulates themes of horror, self-harm, and gore, and is classified as ``\textit{\levelBword}''.

% \par Furthermore, the ``\textbf{Subject Description}'' in a Stable Diffusion prompt can also encompass harmful activities or actions. This includes illegal actions, defamation, and other detrimental behaviors. Such content is referred to as ``\textit{\levelCword}''.

% \par Finally, beyond individual harmful elements, a combination of several elements above can increase the risk. For instance, the depiction of certain celebrities performing specific actions could result in more severe harm than individual harmful elements alone. We term these combinations of various detrimental elements as ``\textit{\levelDword}''.

% We summarized the motivation for social platforms to moderate content and the detailed categories of moderated content for different social platforms.




% court orders, written requests from national and local
% government agencies, and requests from law enforcement

% Now we focus on the motivation for social platforms to moderate content. Such motivations mainly come from the aspects below:

% \par \textbf{Government Legal Requirements}: First of all, governments have laws to request content moderation on social platforms. In the US, FOSTA-SESTA creates a new exception to Section 230 which protects platforms from legal liability for engaging in content moderation, stating that Section 230 does not apply to civil and criminal charges of sex trafficking or conduct that `promotes or facilitates prostitution.' This means that if a third party is found to be advertising the sex trade (including consensual sex work) on its platform, the platform will be held liable. The French government also has established a law to request Twitter to prohibit content that provides false information about voting or registering to vote~\cite{twitterFrance:Online}. Europe Union also regulates Digital Service Acts to regulate the content published on social platforms~\cite{twitterEU:Online}. We summarize different countries' regulations for content moderation in Table. \ref{tab:lawStudy}. Other than the general law, there are some special regulations for content moderation.
% \par \textbf{Copyright Requirements}: At the same time, platforms also have the need to moderate content based on copyright requirements. The Digital Millennium Copyright Act (DMCA) stipulates that if a copyright owner complains about infringement by others, the relevant platform must prohibit access to the infringing work to avoid liability. Google~\cite{google:Online} and other related platforms have also set up a complete process for delisting copyright-infringing content.
% \par \textbf{Law Enforcement Agency Requirements}: Platforms also continuously receive content removal requests from all levels of government through a variety of channels (e.g., court orders, written requests from national and local government agencies, and requests from law enforcement officials). TikTok even provides a unified interface for cooperating with law enforcement to establish content moderation~\cite{tiktok:Online}.
% \par \textbf{GDPR Privacy Regulation}: The General Data Protection Regulation (GDPR) also gives individuals the right to ask for their data to be deleted and organizations do have an obligation to do so. According to GDPR's request, organizations are expected to take reasonable steps (for example technical measures) to inform other websites that a particular individual has requested the erasure of their personal data.

% \subsubsection{What Content Social Platforms Want to Moderate?}
\label{sec:understanding:platform:what}
% \par Then we analyzed the social platforms' regulations and guidelines' detailed content moderation rules about what content is harmful and make a summary in Table \ref{tab:communityStandards}.
% \par Among the 6 famous social platforms we analyzed, Twitter, Facebook and Youtube offer very strong and detailed content moderation. Furthermore, all of them provide detailed examples about the content they want to moderate. While other 3 social platforms's content moderation is very weak. They also do not provide detailed examples to state the content they want to moderate.
% \par From our analysis we can also conclude the content that social platforms want to moderate:
% \par \textbf{Misinformation}: Almost all the platforms care about the misinformation. News about misinformation content on platforms that can influence the market, social opinions, and even elections emerge endlessly. 
% \par \textbf{Violence \& Hate Behavior \& Bully \& Harrass}: Social platforms also care about moderate these contents. Since certain contents have been utilized to spread hate, and discrimination and even directly used to attack certain persons, the harm of such content is self-evident.
% \par \textbf{Violent Content (Terrorism, Militarism)}: Since social platforms have become a battlefield for public opinion, a large number of violent organizations and terrorists have begun to use social networking sites to promote terrorism and militarism. They will even use social platforms to recruit new members. In order to prevent their platforms from becoming a communication tool for these organizations, social platforms have also moderated such content.
% \par \textbf{Adult Nudity}: Some platforms have relatively strict censorship policies on adult nudity, while some platforms allow restricted dissemination of adult nudity content (with the consent of the nude person). It is undeniable that the spread of nudity is harmful to a certain extent, especially when vulnerable groups, such as children, will be greatly affected by pornographic content.
% \par \textbf{Illegal Items and Service}: The use of social platforms to peddle and disseminate illegal goods and services is a common practice. Criminals can sell their items faster. In order to prevent their platforms from becoming platforms for selling illegal items, most platforms also moderate this type of content more intensively.
% \par \textbf{Self-Harm}: Self-harm is also a common harmful content spread on social platforms. Some organizations even use platforms to spread a culture of self-harm (Blue Whale). Some victims will also use the platform to spread their self-harm pictures (eating disorders, pictures of cutting themselves with sharp objects) or self-harm emotions.
% \par \textbf{Child Sex \& Abuse}: Child pornography and abuse are also a focus of the platform. In order to prevent pedophiles and illegal elements from spreading and trading child pornography and abuse content through social platforms, almost all platforms have adopted very strict child pornography censorship policies.
% \par \textbf{Graphic content (Bloody, Gore, Horror)}: Graphic content (gore, gore, horror) often causes a greater mental impact on vulnerable people. If children see these contents, they will have a great psychological impact, which will have a great impact on the children's mental health and growth.
% \par \textbf{Copyright}: The platform also takes copyright-infringing content very seriously. Indulgence of copyright-infringing content often leads to the platform itself becoming the target of copyright litigation, so the platform often strictly moderates copyright-infringing content and behavior.
% \par \textbf{Personal Privacy}: Some posted content may also violate personal privacy. For example, by including other people's faces in posted photos, or posting other people's privacy-related content, half of the platforms also conduct large-scale moderation of content that violates privacy.
% \par \textbf{Weapon Content}: Due to different policies in different regions, weapons-related content is often not the focus of platforms’ censorship, and most platforms do not have censorship strategies for weapons-related content. A small number of strategies mainly target the illegal sale of weapons on the platform and even disseminate the manufacturing process of weapons.




\sssec{Model editing}. The lightweight model editing approaches emerge quickly since the growth of model training costs makes retraining impossible. An intuitive approach is to fine-tune the model using the new data \cite{zhu2020modifying}. Another example is to develop a new model to store new knowledge and utilize a scope classifier to route \cite{mitchell2022memory}. \cite{geva2020transformer} adopts a more accurate process to edit each neuron by observing the influence of each neuron.

\par However, these methods do not meet the requirement of content moderation in Stable Diffusion since these approaches can not achieve free load and offload of the moderation policy since they require the whole fine-tuning process. They can not achieve the free composability of different moderation policies freely. Unlike the previous model editing method, task vectors \cite{ilharco2022editing} enable the model editing in a composable way through the combination of different task vectors. The key observation of \sysname is to achieve a composable and free-loaded moderation process through task vectors \cite{ilharco2022editing}. 


\subsection{Defend Adversarial Examples}

\sssec{Method.} We evaluate \sysname's defense ability against previous state-of-the-art automated attack framework SnearkyPrompt \cite{yang2023sneakyprompt} which is based on RL. We deployed the framework using the code from github \footnote{\url{https://github.com/Yuchen413/text2image_safety}}. Furthermore, we compared \sysname with four current content moderation methods in TTI model:
\begin{itemize}[leftmargin=*,itemsep=-4pt]
    \item \textit{Text-match}: this is a text-based safety filter that blocks the sensitive prompts that contain the sensitive keywords from a predefined dictionary \footnote{\url{https://github.com/rrgeorge-pdcontributions/NSFW-Words-List/blob/master/nsfw_list.txt}}.
    \item \textit{Text-classifier}: this is an open-source, textbased safety filter \footnote{\url{https://huggingface.co/michellejieli/NSFW_text_classifier}} on HuggingFace, which adopts a binary classifier fine-tuned on DistilBERT with the Reddit posts containing NSFW content.
    \item \textit{Image-classifier}: this is an open-source, image-based safety filter \footnote{\url{https://github.com/lakshaychhabra/NSFW-Detection-DL}} that classifies images as either porn, sexy, or normal and blocks contents related to the former two.
    \item \textit{Image-clip-classifier}: this is an opensource, image-based safety filter with a binary classifier \footnote{\url{https://github.com/LAION-AI/CLIP-based-NSFW-Detector}} trained with the CLIP image embedding of an NSFW image dataset \footnote{\url{https://github.com/alex000kim/nsfw_data_scraper}}.
\end{itemize}
Then we compare all the content moderation methods against SneakyPrompt. We compute the bypass rate as the number of adversarial prompts that bypass a safety filter divided by the total number of adversarial prompts.

\begin{figure}[htb!]
\centering
\includegraphics[width=0.48\textwidth]{figs/exp-SneakyPrompt.pdf}
\caption{
\sysname can achieve nearly zero bypass rate against SneakyPrompt, which proves it is a better content moderation method compared with previous content moderation method in TTI model.
}
\label{fig:jailbreak}
\end{figure}

\sssec{Results.} The results shown in Fig. \ref{fig:jailbreak} proved that \sysname outperformed previous content moderation methods greatly. Both text match and text classifier moderation methods perform badly with 100\% bypass rate. Image classifier and image-clip classifier achieved a better performance but still got a bypass rate over 60\%. However, \sysname achieved nearly 0\% of bypass rate which indicated its robustness against adversarial examples. This was due to that \sysname directly modified the model weight rather than just detecting on prompt input or image output.

%Administrators of the online TTI model have large requirements to moderate the TTI model to align with the online platforms' policy. We designed \sysname to align the online text-to-image platform's model with its content ethical policy. Users of such platforms may misuse the model to generate harmful content. For instance, teenagers may accidentally generate inappropriate content detrimental to their mental well-being~\cite{scheuerman2021framework}. Malicious users can exploit the service to create harmful content to spread fake news and harmful thoughts (for example, users have used Stable Diffusion to create fake news of Macron and Trump to spread fake political memes)~\cite{scheuerman2021framework}. To mitigate such harm, Governments have established some laws and regulations to regulate the misuse of online text-to-image models. Following these laws and regulations, online text-to-image service providers are expected and required to conduct content moderation policies to prevent users' misuse of generative AI services.

%\par Our attacker model focuses on the users who intend to produce inappropriate content using the online text-to-image service. We make the following assumptions: (1) \textit{Limited access:} Users can only access the TTI service through the online API, without access to view or edit the model parameter. (2) \textit{Reliable training process:} The training samples are collected and controlled by the platform itself. Attackers can not access or edit the training samples (e.g., poisoning attacks). 

%\par Existing solutions of the platforms use the safety filters to filter the sensitive input prompt or output images \cite{rando2022redteaming}. However, these solutions do not offer the fine-grained and extensive content moderation that meets the needs of various stakeholders. Also, since the existing solutions still leave the weight space of the TTI model unmodified, multiple attack frameworks that use adversarial examples have successfully bypassed them \cite{yang2023sneakyprompt, ba2023surrogateprompt}. \cite{yang2023sneakyprompt} utilized an iterative process to find the boundary space of the safety filters, and \cite{ba2023surrogateprompt} used an LLM-based prompt description process to avoid the sensitive prompt detection. All of these bypass methods benefit from the boundary space of safety filters and unmodified model weight.



%\subsection{Understanding Regulators' Requirements on Harmful Images}
%\label{sec:understanding:platform}

%Given the existing regulations for social media content, we first examined content policies on social platforms to understand regulatory requirements for harmful online content.

%\sssec{Method}. First, we reviewed the literature on content moderation in social media~\cite{gillespie2018custodians, roberts2019behind, bateman2021social} and examined community guidelines of common social media platforms, including Twitter~\cite{xPolicy:Online}, Facebook~\cite{facebookPolicy:Online}, YouTube~\cite{ youtubePolicy:Online}, TikTok~\cite{tiktokPolicy:Online}, Instagram~\cite{insPolicy:Online} and Reddit~\cite{redditPolicy:Online}. Specifically, we enumerated the types of restricted content on each platform based on their content policies and conducted comparisons across different platforms. Second, we surveyed the regulations governing social media content in various countries with legal frameworks (e.g., laws, executive orders) ~\cite{USPolicy:online, european2020digital, CNPolicy:online, japanPolicy:online, IndiaPolicy:online, CAPolicy:online, ukPolicy:online}. We applied a similar approach to analyze the requirements of regulators in different regions. 

\begin{figure*}[htb!]
\centering
\includegraphics[width=\textwidth]{figs/cardSorting-2column.png}
\caption{We grouped various potentially harmful content generated by TTI into 18 categories. This coding process was conducted and cross-validated by two authors in the Miro platform~\cite{miro2023:online}.}
\label{fig:coding}
\end{figure*}

\sssec{Results}. 
% complex policies / dynamic policies
\par Our investigation indicates that there is no one-for-all solution to govern all the harmful content.

\par First, the administrators may have different needs of regulation due to the diverse content moderation standards enforced by different platforms. These platforms exhibit variations in the scope and extent of their moderation policies. For example, YouTube is the only platform that explicitly prohibits weapon-related content \cite{youtubePolicy:Online}. Additionally, while most platforms impose restrictions on misinformation, some implement broad prohibitions, such as TikTok's policy against “\textit{misinformation that causes significant harm to individuals, our community, or the larger public regardless of intent}" \cite{tiktokPolicy:Online}. In contrast, platforms like Facebook, Twitter, and YouTube restrict false information only in specific cases, such as when it may lead to violence or electoral disruptions~\cite{ bateman2021social}. Likewise, different regions have their own set of laws and regulations governing online content, potentially varying in both scope and the enforcement of moderation. Administrators must navigate this complex web of regulations to ensure compliance with region-specific concerns.

\par Second, the demand for content moderation is dynamic and subject to change. Regulatory requirements may continually adapt to evolving circumstances and respond to new needs arising from public opinion events. For example, Canada initially confined the scope of content moderation to five specific categories \cite{CAPolicy:online}. Nevertheless, many experts have proposed expanding the range of harms to address a broader range of issues \cite{CAPolicy:online}.


\subsection{Analyzing AI-generated Harmful Content}
\label{sec:understanding:GenAI}
Based on the analysis of regulatory requirements on social media, we explored the need for moderating AI-generated images and identified two key challenges.

\sssec{Method}. To explore the potential risks associated with content generated by Text-to-Image (TTI) services, we collected a dataset of 153 prompts from various sources, including social media platforms, the I2P dataset \cite{schramowski2023safe}, and the brainstorming. Two researchers independently reviewed and categorized these prompts, developing a comprehensive codebook to classify the types of harmful content identified (see Appendix, Fig. \ref{fig:coding}). To evaluate the necessity for content moderation, we mapped each identified category of harmful content to relevant moderation requirements as discussed in \S \ref{sec:understanding:platform}, resulting in the identification of 20 distinct categories of harmful content, each associated with specific regulatory compliance (see Table. \ref{tab:what+why}). Subsequently, we experimented with these prompts using a locally deployed Stable Diffusion \cite{rombach2022high}, to identify the potential risks posed by the images generated. These risks were then classified into six primary categories (detailed in Table \ref{tab:harmType}). Finally, to measure the efficacy of content moderation practices on current online TTI platforms, we submitted the collected prompts to these platforms to examine their adherence to established content moderation regulations.

\sssec{Results}. We make the following key observations. First, most existing models on these online \textbf{TTI platforms do not fit the regulatory requirements} outlined in \S \ref{sec:understanding:platform}. As shown in Appendix Table. \ref{tab:Platform}, certain harmful content forbidden by the regulations can still be generated on these platforms. Current content moderation on these platforms is mostly only equipped with prompt-level or image-level content moderation methods which can not defend against state-of-the-art bypass methods.

Second, \textbf{the open-vocabulary nature of prompts} makes it challenging to govern AI-generated content with policies based on a predetermined set of rules. The open-ended prompt allows for a wide range of concepts, resulting in a vast output space with numerous possibilities. Further, harmful AI-generated content manifests in various forms, making it difficult to exhaustively enumerate within predefined categories. Consequently, we need to formulate open-vocabulary policies based on natural language to accommodate diverse possibilities within the prompt space.

\haojian{This paragraph is very important! The current argument is not strong enough!}
Third, AI-generated images need \textbf{fine-grained} and suitable moderation. The moderation should also be conditional but not one-size-fits-all (e.g., Fig. \ref{fig:example-3}, Tom Hanks advertise McDonald should be moderated, but Tom Hanks should not be moderated). One-size-fits-all moderation will negatively impact the generation of benign content related to the moderated content, making users unsatisfactory. Multiple moderation methods are required to moderate in a suitable manner that minimizes interference with the content and preserves the original semantics, as excessive content moderation may lead to user frustration and aversion~\cite{gillespie2018custodians}. Multiple moderation methods can be used, like removing, mosaicking, and replacing the harmful content. Different methods have different moderation effects on the content. Mosaicing and blocking sensitive areas have limited effectiveness, as users can still infer content from the remaining parts of the generated images~\cite{yang2023sneakyprompt}, and it can degrade visual quality. For instance, adding mosaic to the nude part of the body-exposure images will not make the users unaware of the content, but may inspire them to imagine more. However, they can be used in some more slightly harmful content, such as misinformation. The choice of content moderation methods largely depends on the context. For instance, when addressing images that violate copyright, we should just remove the violative content (e.g., Mickey Mouse in Fig. \ref{fig:example-2}). In cases involving violent content, the moderation approach should mitigate the content severity rather than blocking completely, with intervention only when the harm of the content is severe.

\begin{table*}[]\small
\begin{tabular}{|c| p{3cm} | p{6.5cm}| p{5cm}|}
\hline

\# & \textbf{Purpose} & \textbf{Examples} & \textbf{Reasons for Content Moderation}\\
\rowcolor{gray!10}
\hline \hline
1 &
 Horror & Unrealistic body image, Disturbing and gruesome scenes & Legal Requirements~\cite{CNPolicy:online}\\ 
% \hline
2 & Abuse & Controlling or coercive behaviour, Manipulative and emotionally abusive content
& Legal Requirements~\cite{ukPolicy:online, japanPolicy:online, IndiaPolicy:online, european2020digital}

Government Requests~\cite{USPolicy:online} \\ 
% \hline
\rowcolor{gray!10}
3 & Gore & Graphic crime scenes, Detailed surgical procedures & Legal Requirements~\cite{CNPolicy:online} \\ 
% \hline
4 & Violence & Incitement of violence, Glorification of violence
 &  Legal Requirements~\cite{CNGenAIPolicy:online, CNPolicy:online, ukPolicy:online, european2020digital, CAPolicy:online}\\ 
% \hline
\rowcolor{gray!10}
5 & Sexual Content & Sexual exploitation, Adult nudity, Sexual violence
% Assault Revenge porn
& Legal Requirements~\cite{CNGenAIPolicy:online, CNPolicy:online, ukPolicy:online, japanPolicy:online, IndiaPolicy:online, european2020digital, CAPolicy:online} \\ 
% \hline
6 & Self-Harm & Self-inflicted wounds, Suicidal depictions
 & Legal Requirements~\cite{ukPolicy:online, IndiaPolicy:online} \\ 
% \hline
\rowcolor{gray!10}
7 & Piracy & Counterfeit goods with logos, Copyright and trademark infringement & 
% Copyright requirements (DMCA)
Legal Requirements ~\cite{CNGenAIPolicy:online, IndiaPolicy:online, european2020digital}

Government Requests~\cite{USPolicy:online}

Content delistings due to copyright~\cite{google:Online}
\\ 
% \hline
8 & Illegal Activities & Illegal drugs or weapons, Money laundering or gambling, Psychotropic substances & Legal Requirements ~\cite{CNGenAIPolicy:online, CNPolicy:online, ukPolicy:online, japanPolicy:online, IndiaPolicy:online, european2020digital}  \\ 
% \hline
\rowcolor{gray!10}
9 & Disinformation & Fake images of fabricated events, False advertising, Fraud and scams & Legal Requirements~\cite{CNGenAIPolicy:online, CNPolicy:online, ukPolicy:online, japanPolicy:online, IndiaPolicy:online, european2020digital}

Government Requests~\cite{USPolicy:online}\\ 
% deceives or misleads the addressee about the origin of the message or knowingly and intentionally communicates any information which is patently false or misleading in nature but may reasonably be perceived as a fact;
% \hline
10 & Unlimited Jokes & Offensive and derogatory humor, Racist or sexist jokes  & Legal Requirements~\cite{CNPolicy:online} \\ 
% \hline
\rowcolor{gray!10}
11 & Defamation  & False accusations, Libelous images harming reputations & Legal Requirements~\cite{CNPolicy:online, CNGenAIPolicy:online, japanPolicy:online, IndiaPolicy:online}\\ 
% \hline
12 & Discrimination/Bias  & % Hate crime, Racially or ethnically objectionable, 
Dehumanization based on race, religion, or ethnicity, Reinforcing biased stereotypes  & Legal Requirements~\cite{CNPolicy:online, CNGenAIPolicy:online, ukPolicy:online, european2020digital}

Government Requests~\cite{USPolicy:online}\\ 
% \hline
\rowcolor{gray!10}
13 & Insulting Beliefs & Offensive depictions of religious figures, Disparaging specific beliefs & Legal Requirements~\cite{CNGenAIPolicy:online, CNPolicy:online, IndiaPolicy:online}\\ 
% \hline
14 & Creating Conflicts & Provocative content fueling societal divisions, Portrayals of historical conflicts to incite hostility & Legal Requirements~\cite{CNGenAIPolicy:online, CNPolicy:online, IndiaPolicy:online} \\ 
% \hline
\rowcolor{gray!10}
15 & Political Propaganda & Propaganda promoting extremist ideologies, Misleading political communications influencing public opinions & Legal requirements~\cite{european2020digital}\\ 
% \hline
16 & Terrorism  & Graphic terrorist attacks, Images glorifying acts of terrorism & Legal Requirements~\cite{CNGenAIPolicy:online, CNPolicy:online, ukPolicy:online, european2020digital, CAPolicy:online}\\ 
% \hline
\rowcolor{gray!10}
17 & Children Harm & Child sexual exploitation and abuse, Paedophilia content or predatory behavior 
% image beating, strangling or suffocating by an adult.
& Legal Requirements~\cite{CNPolicy:online, ukPolicy:online, IndiaPolicy:online, european2020digital, CAPolicy:online}

 Government Requests~\cite{USPolicy:online}\\ 
18 & Privacy Breaches & Non-consensual sharing of private content, Leaked training images with actual individuals & The General Data Protection Regulation (GDPR) 

Legal Requirements ~\cite{CNGenAIPolicy:online, CNPolicy:online, japanPolicy:online, IndiaPolicy:online, european2020digital}

Personal Requests\\
\rowcolor{gray!10}
19 & Violation of public order and morals & Indecent public behaviors, Incitement of riots, looting, and vandalism & Legal Requirements~\cite{japanPolicy:online, CNGenAIPolicy:online, CNPolicy:online, IndiaPolicy:online}\\
20 & Threatening national unity and sovereignty & Maps and symbols illustrating the division of a nation, Promoting insurrections and civil uprisings & Legal Requirements~\cite{IndiaPolicy:online, CNGenAIPolicy:online, CNPolicy:online}\\
% threatens the unity, integrity, defence, security or sovereignty of India, friendly relations with foreign States, or public order, or causes incitement to the commission of any cognisable offence or prevents investigation of any offence or is insulting other nation;
% \hline
\hline
\end{tabular}%
\caption{We categorized 153 prompts that may generate prompts through GenAI services into 20 content types and enumerated reasons for moderation for each specific type.}
\label{tab:what+why}
\end{table*}

\begin{table*}[htbp]\normalsize
\centering
\begin{tabular}{| p{3.5cm} | p{6cm} | p{5cm} |}
\hline
\textbf{Harm type} & \textbf{Definition} & \textbf{Examples}  \\ 
\hline
\hline

\rowcolor{gray!10}
Emotion
& Content causing psychological distress, often featuring horror, self-harm, or depression, without significant societal impact. 
& Graphic self-harm or suicide content, Physical or emotional abuse, Horror content \\ 

Personal relation
& Content that adversely impacts an individual's public image with negative social outcomes.
& Defamatory content that falsely accuses an individual of misconduct \\

\rowcolor{gray!10}
Inappropriate behavior
& Visuals illustrating individuals involved in negative behaviors or character traits, with the potential to incite imitation if disseminated. 
& Images glamorizing harmful behavior like violence, or illegal activities \\

Social group relation
& Depictions of specific social groups with substantial social repercussions for the group's image. 
& Depictions reinforcing stereotypes and discrimination, Content that undermines the reputation of specific social groups

\rowcolor{gray!10}
Infringement
& Images containing copyrighted material or trademarks, infringing on intellectual property rights. 
& Counterfeit products, AI-generated art reproducing copyrighted artwork or designs\\

Children
& Material that endangers the safety, well-being, or development of minors, such as sexual exploitation, abuse, or violence. 
& Explicit sexual images of minors, Depictions of violence and abuse against children\\
\hline
\end{tabular}%
\caption{We classified the harm brought by harmful AI-generated contents into 6 types.}
\label{tab:harmType}
\end{table*}

\begin{table*}[]\normalsize
\centering
\begin{tabular}{|p{3cm} | M{1.8cm} | M{1.8cm} | M{1.8cm} | M{1.8cm} | M{1.8cm} | M{1.8cm} |}
\hline
\textbf{Purpose} & Removing \levelAword & Replacing \levelAword & Mosaicking \levelAword & Removing \levelBword & Replacing \levelBword & Replacing \levelCword \\
\hline \hline
\rowcolor{gray!10}
Horror & \textcolor{green}{\Checkmark} & \textcolor{green}{\Checkmark} & \textcolor{green}{\Checkmark} & \textcolor{green}{\Checkmark} & \textcolor{green}{\Checkmark} & \textcolor{red}{\XSolidBrush}\\ 
%\hline
Abuse & \textcolor{red}{\XSolidBrush} & \textcolor{red}{\XSolidBrush} & \textcolor{red}{\XSolidBrush} & \textcolor{red}{\XSolidBrush} & \textcolor{red}{\XSolidBrush} & \textcolor{green}{\Checkmark} \\
% \hline
\rowcolor{gray!10}
Gore & \textcolor{red}{\XSolidBrush} & \textcolor{red}{\XSolidBrush} & \textcolor{red}{\XSolidBrush} & \textcolor{green}{\Checkmark} & \textcolor{green}{\Checkmark} & \textcolor{red}{\XSolidBrush} \\
% \hline
Violence & \textcolor{red}{\XSolidBrush} & \textcolor{red}{\XSolidBrush} & \textcolor{red}{\XSolidBrush} & \textcolor{red}{\XSolidBrush} & \textcolor{red}{\XSolidBrush} & \textcolor{green}{\Checkmark} \\
% \hline
\rowcolor{gray!10}
Sexual Content & \textcolor{green}{\Checkmark} & \textcolor{green}{\Checkmark} & \textcolor{green}{\Checkmark} & \textcolor{red}{\XSolidBrush} & \textcolor{red}{\XSolidBrush} & \textcolor{green}{\Checkmark} \\
% \hline
Self-Harm & \textcolor{red}{\XSolidBrush} & \textcolor{red}{\XSolidBrush} & \textcolor{red}{\XSolidBrush} & \textcolor{red}{\XSolidBrush} & \textcolor{red}{\XSolidBrush} & \textcolor{green}{\Checkmark} \\ 
% \hline
\rowcolor{gray!10}
Piracy & \textcolor{green}{\Checkmark} & \textcolor{green}{\Checkmark} & \textcolor{green}{\Checkmark} & \textcolor{red}{\XSolidBrush} & \textcolor{red}{\XSolidBrush} & \textcolor{red}{\XSolidBrush} \\
% \hline
Illegal Activities & \textcolor{green}{\Checkmark} & \textcolor{green}{\Checkmark} & \textcolor{green}{\Checkmark} & \textcolor{red}{\XSolidBrush} & \textcolor{red}{\XSolidBrush} & \textcolor{green}{\Checkmark} \\
% \hline
\rowcolor{gray!10}
Disinformation & \textcolor{red}{\XSolidBrush} & \textcolor{red}{\XSolidBrush} & \textcolor{red}{\XSolidBrush} & \textcolor{red}{\XSolidBrush} & \textcolor{red}{\XSolidBrush} & \textcolor{green}{\Checkmark} \\
% \hline
Unlimited Jokes & \textcolor{red}{\XSolidBrush} & \textcolor{red}{\XSolidBrush} & \textcolor{red}{\XSolidBrush} & \textcolor{red}{\XSolidBrush} & \textcolor{red}{\XSolidBrush} & \textcolor{green}{\Checkmark} \\
% \hline
\rowcolor{gray!10}
Defamation & \textcolor{red}{\XSolidBrush} & \textcolor{red}{\XSolidBrush} & \textcolor{red}{\XSolidBrush} & \textcolor{red}{\XSolidBrush} & \textcolor{red}{\XSolidBrush} & \textcolor{green}{\Checkmark} \\
% \hline
Discrimination Bias & \textcolor{green}{\Checkmark} & \textcolor{green}{\Checkmark} & \textcolor{red}{\XSolidBrush} & \textcolor{red}{\XSolidBrush} & \textcolor{red}{\XSolidBrush} & \textcolor{green}{\Checkmark} \\ 
% \hline
\rowcolor{gray!10}
Insulting Beliefs & \textcolor{red}{\XSolidBrush} & \textcolor{red}{\XSolidBrush} & \textcolor{red}{\XSolidBrush} & \textcolor{red}{\XSolidBrush} & \textcolor{red}{\XSolidBrush} & \textcolor{green}{\Checkmark}\\
% \hline
Creating Conflicts & \textcolor{red}{\XSolidBrush} & \textcolor{red}{\XSolidBrush} & \textcolor{red}{\XSolidBrush} & \textcolor{red}{\XSolidBrush} & \textcolor{red}{\XSolidBrush} & \textcolor{green}{\Checkmark} \\
% \hline
\rowcolor{gray!10}
Political Propaganda & \textcolor{red}{\XSolidBrush} & \textcolor{red}{\XSolidBrush} & \textcolor{red}{\XSolidBrush} & \textcolor{red}{\XSolidBrush} & \textcolor{green}{\Checkmark} & \textcolor{green}{\Checkmark} \\
% \hline
Terrorism & \textcolor{green}{\Checkmark} & \textcolor{green}{\Checkmark} & \textcolor{red}{\XSolidBrush} & \textcolor{red}{\XSolidBrush} & \textcolor{red}{\XSolidBrush} & \textcolor{green}{\Checkmark} \\
% \hline
\rowcolor{gray!10}
Children Harm & \textcolor{red}{\XSolidBrush} & \textcolor{red}{\XSolidBrush} & \textcolor{red}{\XSolidBrush} & \textcolor{red}{\XSolidBrush} & \textcolor{red}{\XSolidBrush} & \textcolor{green}{\Checkmark} \\
%\hline
Privacy Breaches & \textcolor{green}{\Checkmark} & \textcolor{green}{\Checkmark} & \textcolor{green}{\Checkmark} & \textcolor{red}{\XSolidBrush} & \textcolor{red}{\XSolidBrush} & \textcolor{red}{\XSolidBrush} \\
\rowcolor{gray!10}
Violation of public order and morals & \textcolor{red}{\XSolidBrush} & \textcolor{red}{\XSolidBrush} & \textcolor{red}{\XSolidBrush} & \textcolor{red}{\XSolidBrush} & \textcolor{red}{\XSolidBrush} & \textcolor{green}{\Checkmark} \\
Threatening national unity and sovereignty & \textcolor{red}{\XSolidBrush} & \textcolor{red}{\XSolidBrush} & \textcolor{red}{\XSolidBrush} & \textcolor{red}{\XSolidBrush} & \textcolor{red}{\XSolidBrush} & \textcolor{green}{\Checkmark} \\
\hline\hline
\end{tabular}%
\caption{For each purpose category, we summarized which of the six moderation methods suit its moderation best.}
\label{tab:type+method}
\end{table*}


\begin{table*}[]
\resizebox{\textwidth}{!}{%
\begin{tabular}{|p{2.5cm}|M{1.6cm}|M{1.6cm}|M{1.6cm}|M{1.6cm}|M{1.6cm}|M{1.6cm}|M{1.6cm}|}
\hline
Platform & Dream Studio & Playground & GetImg.AI & leonardo.ai & dezgo & Picso & Stablebility.AI \\ \hline \hline

\rowcolor{gray!10}
Horror & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} \\
%\hline
Abuse & \textcolor[RGB]{0,220,0}{\XSolidBrush} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor[RGB]{0,220,0}{\XSolidBrush} & \textcolor[RGB]{0,220,0}{\XSolidBrush} \\
% \hline
\rowcolor{gray!10}
Gore & \textcolor[RGB]{0,220,0}{\XSolidBrush} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor[RGB]{0,220,0}{\XSolidBrush} & \textcolor[RGB]{0,220,0}{\XSolidBrush} \\
% \hline
Violence & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor[RGB]{0,220,0}{\XSolidBrush} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor[RGB]{0,220,0}{\XSolidBrush} \\
% \hline
\rowcolor{gray!10}
Sexual Content & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} \\
% \hline
Self-Harm & \textcolor[RGB]{0,220,0}{\XSolidBrush} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor[RGB]{0,220,0}{\XSolidBrush} & \textcolor[RGB]{0,220,0}{\XSolidBrush} \\
% \hline
\rowcolor{gray!10}
Piracy & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} \\
% \hline
Illegal Activities & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} \\
% \hline
\rowcolor{gray!10}
Disinformation & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} \\
% \hline
Unlimited Jokes & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} \\
% \hline
\rowcolor{gray!10}
Defamation & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} \\
% \hline
Discrimination/Bias & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} \\
% \hline
\rowcolor{gray!10}
Insulting Beliefs & \textcolor[RGB]{0,220,0}{\XSolidBrush} & \textcolor[RGB]{0,220,0}{\XSolidBrush} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor[RGB]{0,220,0}{\XSolidBrush} \\
% \hline
Creating Conflicts & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} \\
% \hline
\rowcolor{gray!10}
Political Propaganda & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} \\
% \hline
Terrorism & \textcolor{red}{\Checkmark} & \textcolor[RGB]{0,220,0}{\XSolidBrush} & \textcolor[RGB]{0,220,0}{\XSolidBrush} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor[RGB]{0,220,0}{\XSolidBrush} \\
% \hline
\rowcolor{gray!10}
Children Harm & \textcolor[RGB]{0,220,0}{\XSolidBrush} & \textcolor[RGB]{0,220,0}{\XSolidBrush} & \textcolor[RGB]{0,220,0}{\XSolidBrush} & \textcolor[RGB]{0,220,0}{\XSolidBrush} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor[RGB]{0,220,0}{\XSolidBrush} \\
%\hline
Privacy Breaches & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} \\
\rowcolor{gray!10}
Violation of public order and morals & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} \\
%\hline
Threatening national unity and sovereignty & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} & \textcolor{red}{\Checkmark} \\
\hline \hline
\end{tabular}%
}
\caption{We summarize 7 popular GenAI online platforms. According to the card sorting results we do in Table. \ref{tab:what+why}, we test all the 7 GenAI platforms to see if they can generate certain types of harmful content.}
\label{tab:Platform}
\end{table*}

\begin{table*}[]\normalsize
\centering
\begin{tabular}{|p{0.5cm}|p{2cm}|p{2cm}|p{4cm}|p{6.5cm}|}
\hline
ID\# & Method & Simulation Target & Policy & Policy Context \\
\hline \hline

\rowcolor{gray!10}
1
&
Replace object
&
Mickey Mouse
&
\raisebox{-.9\height}{\begin{minipage}[b]{4cm} 
content:
\par \hspace{0.2cm}\levelAword:\levelA{``Mickey Mouse"}
\par \hspace{0.2cm}\hspace{0.5cm}$\Rightarrow$\levelA{``Mouse"}
\par method=\textcolor{black}{``Replacing"}
\end{minipage}}
&
The creation of cartoon character images will cause piracy
%&
%Piracy
\\ \hline

2
&
Removing \levelAword
&
Tom Hanks
&
\raisebox{-.9\height}{\begin{minipage}[b]{4cm} 
content:
\par \hspace{0.2cm}\levelAword:\levelA{``Tom Hanks's Face"}
\par method=\textcolor{black}{``Removing"}
\end{minipage}}
&
Malicious creators create insulting images of specific celebrities in order to stigmatize them
%&
%Defamation/ Discrimination
\\ \hline

\rowcolor{gray!10}
3
&
Removing \levelAword
&
Snake
&
\raisebox{-.9\height}{\begin{minipage}[b]{4cm} 
content:
\par \hspace{0.2cm}\levelAword:\levelA{``Cat"}
\par method=\textcolor{black}{``Blocking"}
\end{minipage}}
&
Teenagers will mistakenly create images of scary creatures like snakes, centipedes, etc. Since participants cannot also see such images, we used cat as simulation content
%&
%Horror
\\ \hline

4
&
Replacing \levelBword
&
Greasy tentacle style
&
\raisebox{-.9\height}{\begin{minipage}[b]{4cm} 
content:
\par \hspace{0.2cm}\levelBword:\levelB{``Cartoon Style"}
\par \hspace{0.2cm}\hspace{0.5cm}$\Rightarrow$\levelA{``Realistic Style"}
\par method=\textcolor{black}{``Replacing"}
\end{minipage}}
&
Teenagers may mistakenly create greasy tentacle-style pictures, which may have an impact on their mental health; since participants cannot also see such images, we use the moderation of ``Cartoon Style" to simulate the moderation of such images.
%&
%Self-Harm/ Horror
\\ \hline

\rowcolor{gray!10}
5
&
Removing \levelBword
&
Bloody Arm
&
\raisebox{-.9\height}{\begin{minipage}[b]{4cm} 
content:
\par \hspace{0.2cm}\levelAword:\levelA{``Arm"}
\par \hspace{0.2cm}\levelBword:\levelB{``Sweaty}
\par method=\textcolor{black}{``Removing"}
\end{minipage}}
&
Teenagers may mistakenly create pictures of bleeding arms; since participants cannot also see such images, we simulated the moderation of such images by moderating sweaty arms.
%&
%Self-Harm/ Horror
\\ \hline

6
&
Replacing \levelCword
&
Einstein kiss people
&
\raisebox{-.9\height}{\begin{minipage}[b]{4cm} 
content:
\par \hspace{0.2cm}\levelAword:\levelA{``Einstein"}
\par \hspace{0.2cm}\levelCword:\levelC{``Kiss"}
\par \hspace{0.2cm}\hspace{0.5cm}$\Rightarrow$\levelA{``Hug"}
\par method=\textcolor{black}{``Replacing"}
\end{minipage}}
&
In the opinion of some people, kissing is more inappropriate for children than hugging and should not be shown in front of young children.
%&
%Illegal Activities/ Violence
\\ \hline\hline
\end{tabular}
\caption{Six moderated models we offered for attack study in Sec. \ref{sec:eval:attack}. Policy type denoted the moderation method of the policy. The simulation target denoted the moderation target the policy is aimed to simulate (it was not the real moderation target in the policy due to its harm, so we replaced it with likely content in the policy). The policy denoted the moderation policy used to moderate the model. And the policy context denoted the context of the policy including why we need to moderate it.}
\label{tab:atk_study-2:moderated_models}
\end{table*}

\begin{table*}[]
%\resizebox{0.48\textwidth}{!}{%
\centering
\begin{tabular}{|p{2.1cm}|p{1.5cm} |p{0.8cm}|p{0.8cm}|p{0.8cm}|p{0.8cm}|p{0.8cm}|p{0.8cm}|p{0.8cm}|p{0.8cm}|p{1.5cm}|}%{lllllll}
\hline

\textit{\textbf{Participant}} 
& \textit{\textbf{SUS}}
& \textit{\textbf{T1}} % 米奇老鼠
& \textit{\textbf{T2}} % 爱因斯坦的脸
& \textit{\textbf{T3}} % 血淋淋的
& \textit{\textbf{T4}} % 黑暗的、阴郁的
& \textit{\textbf{T5}} % 自刎
& \textit{\textbf{T6}} % 竖中指
& \textit{\textbf{T7}} % 爱因斯坦竖中指
& \textit{\textbf{T8}} % 血淋淋的手臂
& \textit{\textbf{Avg.}}
\\

\hline
\hline

\multirow{2}*{P1} & 62.5 & & 1/1.23 & 1/0.52 & 1/0.47 & & 2/2.15 & & & 1.25/1.09 \\ % Yukun Jiang
&  & & \XSolidBrush & \XSolidBrush & \XSolidBrush & & \XSolidBrush & & & \\ % Yukun Jiang
\hline
\multirow{2}*{P2} & 67.5 & 1/0.67 & & 1/1.13 & & 1/0.89 & & 1/0.67 & & 1/0.84 \\ % Yuzhou Fang
&  & \XSolidBrush & & \XSolidBrush & & \XSolidBrush & & \XSolidBrush & & \\ % Yuzhou Fang
\hline
\multirow{2}*{P3} & 85.0 & & & 7/4.23 & & 2/1.43 & 4/3.21 & 2/0.91 & & 3.75/2.45 \\ % Qiao Yu
&  & & & \XSolidBrush & & \XSolidBrush & \XSolidBrush & \XSolidBrush & & \\ % Qiao Yu
\hline
\multirow{2}*{P4} & 72.5 & & & & 2/1.13 & 1/0.86 & 2/0.87 & 2/1.23 & & 1.75/1.02 \\ % Yuzhuo Liu
&  & & & & \XSolidBrush & \XSolidBrush & \XSolidBrush & \XSolidBrush & & \\ % Yuzhuo Liu
\hline
\multirow{2}*{P5} & 42.5 & & 1/0.76 & & 1/1.76 & & 1/0.97 & & 4/4.23 & 1.75/1.93 \\ % Tong Liu
&  & & \XSolidBrush & & \XSolidBrush & & \XSolidBrush & & \XSolidBrush & \\ % Tong Liu
\hline
\multirow{2}*{P6} & 92.5 & & & 1/0.92 & 1/0.66 & 1/0.87 & & 1/1.27 & & 1/0.93 \\ % Yuqiang Sun
&  & & & \XSolidBrush & \XSolidBrush & \XSolidBrush & & \XSolidBrush & & \\ % Yuqiang Sun
\hline
\multirow{2}*{P7} & 87.5 & & 4/4.76 & & 3/2.21 & 4/3.12 & & 3/2.15 & & 3.5/3.06 \\ % Jianhui Li
&  & & \XSolidBrush & & \XSolidBrush & \XSolidBrush & & \Checkmark/10 & &  \\ % Jianhui Li
\hline
\multirow{2}*{P8} & 95.0 & 1/1.23 & 1/0.54 & & & & & 1/2.31 & 1/2.21 & 1/1.57 \\ % Changhao Wang
&  & \XSolidBrush & \XSolidBrush & & & & & \XSolidBrush & \XSolidBrush &  \\ % Changhao Wang
\hline
\multirow{2}*{P9} & 90.0 & 4/3.12 & & 2/3.01 & 2/1.56 & 3/2.95 & & & & 2.75/2.66 \\ % Huaisen Tian
&  & \Checkmark/10 & & \XSolidBrush & \XSolidBrush & \XSolidBrush & & & & \\ % Huaisen Tian
\hline
\multirow{2}*{P10} & 97.5 & 2/3.14 & & 4/4.21 & 1/2.13 & & & 2/4.12 & & 2.25/3.40 \\ % Yuan Luo
&  & \XSolidBrush & & \XSolidBrush & \XSolidBrush & & & \XSolidBrush & & \\ % Yuan Luo
\hline
\multirow{2}*{P11} & 80.0 & 4/2.91 & 2/1.35 & & & 1/1.67 & & 3/2.65 & & 2.5/2.15 \\ % Pei Nie
&  & \XSolidBrush & \XSolidBrush & & & \XSolidBrush & & \XSolidBrush & &  \\ % Pei Nie
\hline
\multirow{2}*{P12} & 95.0 & 1/0.65 & 4/3.65 & 3/2.16 & & & & & 3/4.12 & 2.75/2.65 \\ % Siyan Xue
&  & \XSolidBrush & \XSolidBrush & \Checkmark/9 & & & & & \Checkmark/6 & \\ % Siyan Xue
\hline
\multirow{2}*{P13} & 67.5 & 3/1.24 & & 3/2.13 & 3/2.16 & & 4/2.76 & & & 3.25/2.07 \\ % Yuxiang Guo
&  & \XSolidBrush & & \Checkmark/9 & \XSolidBrush & & \XSolidBrush & & &  \\ % Yuxiang Guo
\hline
\multirow{2}*{P14} & 95.0 & 5/3.23 & 2/1.54 & & 1/0.87 & 3/2.14 & & & & 2.75/1.94 \\ % Zihao Wei
&  & \Checkmark/7 & \XSolidBrush & & \XSolidBrush & \XSolidBrush & & & & \\ % Zihao Wei
\hline
Avg. Attempts & 80.7 & 2.625 & 2.14 & 2.75 & 1.67 & 2 & 2.6 & 1.88 & 2.67 & 2.29 \\
\hline
Avg. Time (min.) & 80.7 & 2.02 & 1.97 & 2.29 & 1.44 & 1.74 & 1.99 & 1.91 & 3.52 & 2.11 \\
\hline
\hline
\end{tabular}
%}
\caption{We record all the participants' SUS scores, policy authoring attempts number, and authoring time cost of each participant in his corresponding 1st row in this table. Each participant's authoring is recorded as ``attempt number/time cost(min)'' in each cell. In the 2nd row for each participant, we recorded their bypass attempts. \XSolidBrush denotes failed bypass, and ``\Checkmark/No. Attempts'' denotes the successful bypass the the number of attempts to bypass.}
\label{tab:admins:cost}
\end{table*}

\sssec{Principle of linear interpolation.}
Previous works discussed linear interpolation's potential application in model editing \cite{ilharco2022patching}.
They found that the linear interpolating would not decrease the model performance substantially.
Furthermore, the linear interpolating combination of two neural network weights can achieve nearly the same accuracy with the two networks' ensemble predictions.

\par \textbf{Preserve performance on unrelated tasks.} They found the linear interpolating of two neural network weights that share part of their optimization trajectory (e.g., two neural networks finetuning from the same pretrained model) does not decrease the model performance substantially \cite{ilharco2022patching, frankle2020linear, izmailov2018averaging}.
First of all, \cite{lucas2021analyzing, ilharco2022patching} observed that performance steadily increases on the linear path between a model before and after training. 
This indicates that the performance gains on the finetuning task are attributed to the direction of the linear path from the pretrained to the finetuned model.
Furthermore, \cite{ilharco2022patching} found that linear interpolations between a pretrained model and a finetuned model can preserve accuracy on tasks that are unrelated to finetuning, while greatly improving accuracy on the finetuning task compared to the pretrained model.
This indicates that the accuracy of the finetuning task and unrelated tasks are independent of each other along the linear path between pre-trained and finetuned models

\par \textbf{Achieve approximate performance of ensemble prediction on related tasks.} Besides that, the well-established practice of ensembling predictions proves that the linear combinations of finetuned neural network weights can achieve ensemble learning level accuracy on their finetuned tasks.
\cite{wortsman2022robust} shows that the result from linearly combining the weights of neural networks approximate ensembling their outputs in certain regimes.
This approximation holds whenever the loss can be locally approximated by a linear expansion, referred to as the NTK regime \cite{jacot2018neural}.
Moreover, as shown by \cite{fort2020deep}, this linear expansion becomes more accurate in the later phase of training neural networks, which closely resembles finetuning.
When the approximation holds exactly, weight averaging and ensembles are equivalent \cite{wortsman2022robust}. 


% The SUS test score shows that almost all . We further categorized the participants by expertise in GenAI and content moderation in Fig. \ref{fig:admin_sus_expert}. 

% The results showed that the non-expert gave \sysname\ with a higher score, while the expert gave a lower score. The reason was that expert participants wanted more customized functions.

% \begin{mdframed}[linecolor=black,linewidth=1pt]
%     ``If \sysname\ can provide customized fine-tune prompts rather than we directly use the content expansion, it would be better.'' --- P14, expert in GenAI and a forum manager in content moderation.
% \end{mdframed}

% \begin{mdframed}[linecolor=black,linewidth=1pt]
%     ``I want to have a more automatic process. For instance, I now have a picture that is harmful and needs to be moderated, I want to just input this picture into \sysname, then \sysname\ should automatically generate policy for the picture I want to moderate.'' --- P12, an expert in GenAI and a group manager in content moderation.
% \end{mdframed}

% \par\textbf{Inconsistent Policy Design Among Participants.} We found that even for the same task, the policies designed by different participants were not consistent. For example, for \textit{\textbf{T3:Bloody}}, P6 designed the policy as

% \begin{mdframed}[linecolor=black,linewidth=1pt]
% \textcolor{black}{policy}:
% \par  \hspace{0.5cm}content:\textcolor{black}{``\$content''}
% \par  \hspace{1cm}\levelAword:\textcolor{black}{\$expand(Object)},
% \par  \hspace{1cm}\levelBword:\textcolor{black}{``Bloody''},
% \par  \hspace{1cm}\levelCword:\textcolor{black}{\$expand(Action)},
% \par  \hspace{0.5cm}purpose:\textcolor{black}{``Gore/Horror''}
% \par  \hspace{0.5cm}method:\textcolor{black}{``Removing''}
% \end{mdframed}

% In his policy, he considered moderation content ``Bloody'' as style. And P3 designed the policy as

% \begin{mdframed}[linecolor=black,linewidth=1pt]
% \textcolor{black}{policy}:
% \par  \hspace{0.5cm}content:\textcolor{black}{``\$content''}
% \par  \hspace{1cm}\levelAword:\textcolor{black}{``Blood''$\to$``Green liquid''},
% \par  \hspace{1cm}\levelBword:\textcolor{black}{\$expand(Style)},
% \par  \hspace{1cm}\levelCword:\textcolor{black}{\$expand(Action)},
% \par  \hspace{0.5cm}purpose:\textcolor{black}{``Gore/Horror''}
% \par  \hspace{0.5cm}method:\textcolor{black}{``Replacing''}
% \end{mdframed}

% This was because he considers the moderation content ``Bloody'' as an object. In another task \textit{\textbf{T7:Einstein give the middle finger}}, P4 designed policy uses ``give the middle finger'' as an action to moderate. In another task \textit{\textbf{T6:give the middle finger}}, the policy designed by P13 was:

% \begin{mdframed}[linecolor=black,linewidth=1pt]
% \textcolor{black}{policy}:
% \par  \hspace{0.5cm}content:\textcolor{black}{``\$content''}
% \par  \hspace{1cm}\levelAword:\textcolor{black}{``middle finger''$\to$``thumb''},
% \par  \hspace{1cm}\levelBword:\textcolor{black}{\$expand(Style)},
% \par  \hspace{1cm}\levelCword:\textcolor{black}{\$expand(Action)},
% \par  \hspace{0.5cm}purpose:\textcolor{black}{``Defamation''}
% \par  \hspace{0.5cm}method:\textcolor{black}{``Replacing''}
% \end{mdframed}
% Different participants had different understandings of the same content, and some actions would be understood as objects for moderation.

% \par\textbf{How to use \textit{``Replacing''} Method Effectively?} Some participants found that when running the replacing method if the content before and after the replacement was too different, the model's ability would significantly decrease. For example, for \textit{\textbf{T8:Bloody Arm}}, P12 made an interesting attempt. He replaced the ``Bloody Arm'' with ``the Sweaty Leg''. Although the moderation successfully replaced the Bloody Arm drawn by the model with the Sweaty Leg, it had a significant impact on the effects of other human body-related pictures drawn by the model. In his next attempt, he replaced the Bloody Arm with the Sweaty Arm, resulting in the policy having much less impact on the model's capabilities.

% \par\textbf{Multiple context-based Policy is Better.} For the same content, policies described by multiple contexts performed better than policies described by a single context. For example, in \textit{T8:Bloody Arm}, P7 made two attempts, one to directly describe ``Bloody Arm'' as a single object, and another to decouple it into ``Bloody'' Style and ` `Arm'' Object. According to the image effects generated by the model, the policy used in the second attempt was more effective in preventing the generation of harmful content. This was because in the first attempted policy, the style attribute in the content was not specified, causing the image prompt generated during the content expansion process to be offset, resulting in content that was not bloody arm.
% \qiyu{I did not understand. I think we generate policies based on the part of speech and should avoid this confusion.}

% \begin{comment}
% \begin{table*}[htbp]\normalsize
% \centering
% \begin{tabular}{| p{3cm} | p{6.5cm} | p{5cm} |}
% \hline
% \textbf{Harm type} & \textbf{Definition} & \textbf{Examples}  \\ 
% \hline
% \hline

% \rowcolor{gray!10}
% Emotion
% & Harm to personal emotions, mental state, and mental health.
% & Pictures of self-harm lead teens to self-harm. \\ 

% Personal relation
% & Harm that affects personal social image, reputation, etc.
% & Images of public figures being arrested by police generated by the TTI model. \\

% \rowcolor{gray!10}
% Inappropriate behavior
% & Images of harmful behavior that lead potential viewers to imitate.
% & Images glamorizing harmful behavior like violence, or illegal activities. \\

% Social group relation
% & Depictions of specific social groups with substantial social repercussions for the group's image.
% & Pornographic images generated by the TTI model lead teens to engage in sexual acts. \\

% \rowcolor{gray!10}
% Infringement
% & Infringement of privacy, copyright, portrait rights, etc.
% & Fake pictures of celebrity endorsement products generated by TTI model.\\

% Children
% & Harm to children's mental health and values.
% & TTI model generates child pornographic images.\\

% \rowcolor{gray!10}
% Financial loss
% & Causing property damage to the viewer of the image.
% & TTI model generates fake bill images\\

% \hline
% \end{tabular}%
% \caption{We classified the harm brought by harmful AI-generated content into 7 types.}
% \label{tab:harmType}
% \end{table*}
% \end{comment}


%\begin{figure*}
%\begin{center}
%\fbox{
%\parbox{\textwidth}{
%}
%}
%\end{center}
%\caption{The prompt template for LLM-as-judge rate metrics in evaluation.}
%\end{figure*}

% \begin{comment}

% \end{comment}

\begin{comment}
\begin{prompt}
\begin{mdframed}[linecolor=black,linewidth=1pt]
\par Consider a context-based content as:
\noindent \operator{METHOD} \lbrack \contentKey{obj}:..., \contentKey{sty}:..., \contentKey{act}:...\rbrack\ \operator{BECAUSE} ...

\par In this structure:
\begin{itemize}[leftmargin=*]
\item The \contentKey{obj} context describes certain objects or entities in the moderated content.
\item The \contentKey{sty} context describes harmful styles of moderated content.
\item The \contentKey{act} context describes the action or activity taken by the "object" context.
\item The \operator{BECAUSE} denotes why to moderate the content, and consists of the potential purposes brought by the content.
\item The \operator{METHOD} denotes how to moderate the content, and provides multiple moderation method choices to support fine-grained moderation control.
\end{itemize}
\par For the \operator{BECAUSE}, we provide potential purposes are [Horror, Abuse, Gore, Violence, Sexual Content, Self-Harm, Piracy, Illegal Activities, Disinformation, Unlimited Jokes, Defamation, Discrimination/Bias, Insulting Beliefs, Creating Conflicts, Political Propaganda, Terrorism, Children Harm, Privacy Breaches, Violation of public order and morals, Threatening national unity and sovereignty]. 
\par Now, consider a text-to-image model prompt: "\textcolor{red}{\$prompt}". You need to figure out what harmful content is contained in this prompt (only consider the harmful content, not other unrelated) and state the content as the element-based content structure description I mentioned above. 
\par Return the content description in Python code as obj=Str sty=Str act=Str BECAUSE=List[Str].
\end{mdframed}
\label{prompt:policyGeneration}
\end{prompt}
\end{comment}

0428-1722

% \peiran{In two of the four tasks, participants experimented with the moderated version of the SDXL model selected from Table. \ref{tab:atk_study-2:moderated_models}. The task target was motivating participants to craft bypass prompts to bypass the moderation policy of the moderated version model. Then we assigned them two other tasks, and each shared the same target with one out of the two previous tasks. For example, a participant was given 4 tasks, among the 4 tasks, one original version task and its corresponding moderated task were: bypassing moderated version of SDXL which moderated ``Mickey Mouse'' to draw ``Mickey Mouse'', and making the original version of SDXL draw ``Mickey Mouse''. The order of all the tasks is shuffled, thus the participants do not know which task is original, and which is moderated.}

% Participants were introduced to the basic principles of \sysname\ and shown an example of different images generated by the same prompt before and after review. 
% Each participant then received an account and password that could access our test interface deployed on the public network. Participants were informed of the reward mechanism and then tested. After the test, the participants submitted the pictures to us. After we checked, we confirmed the valid bypass attempts and recorded the number of valid bypass attempts. Finally, we rewarded the participants based on the reward mechanism. Recorded the following information about the bypass:
% \begin{itemize}
%     \item What method is used by participants to successfully bypass the prompt?
%     \item How many prompts does a participant need to use for each successful bypass?
%     \item Can Expert participants spend fewer prompts than normal participants to bypass?
% \end{itemize}

% \par After the experiment was completed, we invited participants who had successfully bypassed it to fill out a questionnaire. The questionnaire content specifically included the following:
% \begin{itemize}
%     \item What other potential ways do participants think to bypass moderation?
%     \item What factors do you think allow certain audit policies to be successfully bypassed?
%     \item What new ways to bypass moderation do you think may emerge in the future?
% \end{itemize}
